Consensus in Blockchain Systems with Low Network Throughput: A Systematic Mapping Study

Blockchain technologies originate from cryptocurrencies. Thus, most blockchain technologies assume an environment with a fast and stable network. However, in some blockchain-based systems, e.g., supply chain management (SCM) systems, some Internet of Things (IOT) nodes can only rely on the low-quality network sometimes to achieve consensus. Thus, it is critical to understand the applicability of existing consensus algorithms in such environments. We performed a systematic mapping study to evaluate and compare existing consensus mechanisms' capability to provide integrity and security with varying network properties. Our study identified 25 state-of-the-art consensus algorithms from published and preprint literature. We categorized and compared the consensus algorithms qualitatively based on established performance and integrity metrics and well-known blockchain security issues. Results show that consensus algorithms rely on the synchronous network for correctness cannot provide the expected integrity. Such consensus algorithms may also be vulnerable to distributed-denial-of-service (DDOS) and routing attacks, given limited network throughput. Conversely, asynchronous consensus algorithms, e.g., Honey-BadgerBFT, are deemed more robust against many of these attacks and may provide high integrity in asynchrony events.

==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/background.tex <==
\section{Background}

%This section provides necessary background information related to the research. In particular, a brief overview of blockchain technology is provided, highlighting its architecture and key characteristics. Then, terminology and important results related to consensus mechanisms are explained. Finally, important security considerations regarding blockchain systems are discussed, based on the reviews of \citet{RN17} and \citet{RN30}. 


%\subsection{Blockchain technology}

%This section provides a brief overview of blockchain technology; what constitutes a blockchain, key characteristics and the role in which consensus algorithms play in blockchain technology. 



%A blockchain is a specific form of Distributed Ledger Technology (DLT) \citep{RN59}, allowing for the geographical replication, sharing and synchronization of data between peers. Blockchain differentiates itself from other types of DLTs, in that the data it contains are organized as a sequence of blocks, as seen in figure \ref{fig:background_chain}. Each block contains a block header, containing header information, as well as some data, e.g. a list of financial transactions. In particular, the block header contains the hash of the block's parent block. The hash acts as an unique identifier of the parent block. Thus,  a sequential linkage of blocks are created, i.e. a chain, from the most recent block, all they way back to the chain's starting block, denoted the genesis block. 


%\begin{figure}[h]
%    \centering
%    \hspace*{-0.6cm}
%    \includegraphics[width=0.55\textwidth]{graphics/blocks.png}
%    \caption{Visualization of linked blocks, constituting a blockchain. Reprinted from \citet{RN58}. }
%    \label{fig:background_chain}
%\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.5\textwidth]{graphics/block.png}
%    \caption{Visualization of single block, containing header information, as well as data in the form of transactions. Reprinted from \citet{RN58}. }
%    \label{fig:background_block}
%\end{figure}

%A representative blockchain block is shown in figure \ref{fig:background_block}, similar to that used in the cryptocurrency Bitcoin \citep{Nakamoto_Bitcoin_POW}. In addition to the parent block reference, the block header may also contain the following information\footnote{The nBits and Nonce fields are specific to that of blockchain system utilizing a Nakamoto style consensus algorithm, popularized by Bitcoin \citep{Nakamoto_Bitcoin_POW}. In blockchain systems utilizing other types of consensus algorithms, these may be omitted.} \citep{RN58}: \begin{itemize}
    %\item \textbf{Block Version}: The specific version of the blockchain system used when generating the block. Used to keep track of protocol changes.
    %\item \textbf{Merkle Tree Root Hash}: A hash tree of the transactions contained in the block. Ensures the integrity of the transactions stored.  
    %\item \textbf{Timestamp}: Block generation time. Given in seconds, universal time, from January 1, 1970. 
    %\item \textbf{nBits}: Target threshold for a valid block hash. Corresponds to the difficulty level of the blockchain system used when the block was generated. 
    %\item \textbf{Nonce}: The hash value used to solve the target threshold, allowing the generation of the block. 
%\end{itemize}

%Key characteristics of blockchain technology is its ability to provide a high degree of security and robustness. By replicating the data stored within the blockchain across multiple nodes, the system may provide higher availability than that of a centralized system. Furthermore, by the use of strong cryptographic mechanism, such as digital signature and cryptographic hash functions, the validity of the data committed to the blockchain may be verified. This may be particularly important in a financial setting, e.g. asserting that the details of the transaction is correct and that the parties involved are who they claim to be.

%In order to ensure the integrity of the data stored within each respective block in the blockchain, a cryptographic mechanism called a \textit{Merkle Tree} may be utilized \citep{RN60}. As shown in figure \ref{fig:background_merkle}, the leaves of the merkle tree correspond to the data stored in the blockchain, e.g. a set of transactions. A cryptographic hash function is then  used to transform the data into a single root hash value, forming a tree structure. Given the avalanche effect of cryptographic hash functions \citep{RN61}, this allows for cost effective ways of detecting damage or adversarial tampering with the data stored in the blockchain. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.4\textwidth]{graphics/merkle_tree.png}
%    \caption{Visualization of a merkle tree used to ensure the integrity of transactions stored in blockchain. Only the root hash value is kept in block header. Reprinted from \citet{Nakamoto_Bitcoin_POW}. }
%    \label{fig:background_merkle}
%\end{figure}

%To ensure consistency of data shared between participants in the blockchain system, a consensus algorithm is used \citep{RN58}. A consensus algorithm provide a means for participants to reach agreement about a set of values, in a decentralized fashion, without necessitating trust between the participants. The consensus algorithm need to be able to protect the system against adversarial attacks, such as tampering with data, delaying of communication or other malicious behavior.

%Popularized by Bitcoin, Proof of work is a commonly used consensus algorithm, based around participants solving a cryptographic puzzle; when generating a new block, the block header need to be smaller than certain difficulty value. By incrementing the nonce value in the block header, the participants, often denoted miners, may do computational work in order to be allowed to generate the next block, often in return of some reward. Given the the use of a cryptographically strong hash function, this is comparable to a lottery and buying tickets; the amount of computational work a participant puts into solving the puzzle corresponds directly to their chance of winning the next block and reward. Which participants who get to generate the next block is therefore randomized. When a participant finds a solution to the puzzle, they generate the block, include the solution nonce value in the block header, and broadcast it to the rest of the network. The remaining participants verify the validity of the block, and if correct, adds it to their local chain. Given that a majority of the computational power of the network is owned by honest participants, the consensus algorithm can provide strong security guarantees in many types of blockchain networks.

% Meta information removed - the information in not necessary, and I dont need to spend time figuring out why the ref is bugged.
%(for further information on consensus in blockchain, see section \ref{subsec:background_consensus} and section \ref{sec:sota_consensus}). 

%Originating from the success of the cryptocurrency Bitcoin, a multitude of new use cases have been proposed for blockchain technology in recent years. In particular, it has been promoted as a way for independent organizations to share data, in a transparent and secure manner. This has lead to a distinction between permissionless and permissioned blockchain systems: \begin{itemize}
%    \item \textbf{Permissionless blockchain}: Anyone may access the blockchain system.
%    \item \textbf{Permissioned blockchain}: Access to the blockchain is regulated. Only approved entities may participate in teh blockchain system.
%\end{itemize}
%In particular, Bitcoin is an example of a permissionless blockchain system, allowing anyone to trade cryptocurrency. Permissioned blockchain systems may only involve a select few participants, e.g. a partnership between medical institutions to share patient data. Utilizing a permissioned blockchain system may have several benefits, in that access is constrained to only certain participants, providing some level of inherent data confidentiality. Furthermore, as participants are authenticated, the blockchain systems may use different consensus algorithms than that of a permissionless system, potentially offering better performance, energy efficiency or other benefits. 



%\subsection{Consensus mechanisms} \label{subsec:background_consensus}

%This section describes core concepts and terminology related to consensus in distributed systems and consensus algorithms. 

%\subsubsection{Safety and Liveness}

%Central to discussing the integrity and security of consensus mechanisms are the properties of \textit{safety} and \textit{liveness}, established by \citet{RN48}. \textit{Safety} means that incorrect operations cannot happen during execution. \textit{Liveness} mean that correct operations will eventually be executed by the system. Safety is comparable to the correctness of the consensus algorithm. In particular, according to the assumptions made by the consensus model, there is no sequence of events in which the system can enter an erroneous state. As an illustrating example, despite the presence of a adversarial environment, the Nakamoto consensus scheme is able to ensure eventual consistency within the Bitcoin network, given that the assumption of an honest majority within the network holds. Conversely, liveness is comparable to the consensus algorithm's ability to make forward progress. While it is essential that the algorithm is correct, if the algorithm cannot provide liveness, it cannot be effectively utilized in a practical setting. As another illustrating example, despite interference from adversarial parties, honest actors participating in the Nakamoto consensus are eventually able to agree upon a set of transactions, given an honest majority within the network. 

%\subsubsection{Fault tolerance}

%It is a desired quality of consensus algorithms that they are able to tolerate faulty nodes. In particular, for the system to gain  robustness from being distributed across multiple nodes, it must be able to reach consensus despite a subset of the nodes having failed. 

%There are numerous types of faults which may be considered in relation to distributed computing systems. In the context of systems affected by an adversarial environment, such as a permissionless blockchain system, one often consider \textit{Byzantine fault tolerance}. A Byzantine fault is a complex type of fault, in which there is imperfect information related to whether a certain node has failed. Derived from the Byzantine General's problem \citep{RN49}, it depicts a situation in which a node may inconsistently appear faulty from the perspective of other nodes of the network; a node A may seem unresponsive to node B, while it may at the same time respond to messages from node C and therefore seem correct from their perspective. Byzantine faults oftentimes is used to model arbitrary or malicious behavior within the network, in which an adversary may choose to not follow protocol, and thus selectively send information, neglect to respond to messages etc. Byzantine fault tolerance is a measure to which degree a distributed system can withstand Byzantine faults within the network.

%Another type of fault tolerance to consider is \textit{crash tolerance} \citep{RN50}. In this simplified model, one consider non-Byzantine types of faults, in that nodes may crash, but may not show arbitrary behavior. While corresponding to a weaker adversarial model, it is representative for many practical settings, specifically towards to that of a private blockchain system. 

%\subsubsection{CAP Theorem}

%A well known limitation towards distributed systems is the CAP theorem \citep{CAP}. The theorem asserts that it is impossible for a distributed system to simultaneously provide the following qualities: \begin{itemize}
%    \item \textbf{Consistency}: All requests received by the system are executed atomically; as if the system was a single entity. 
%    \item \textbf{Availability}: All requests receive non-error responses. 
%    \item \textbf{Partition Tolerance}: The system continues to operate despite an arbitrary number of messages being lost between network nodes.  
%\end{itemize} 

%\citet{CAP} goes on to prove that systems are able to provide 2/3 out of the qualities, in particular AP, CA or CP. In practical systems, where network nodes are geographically distributed and network partitioning is a definite possibility (e.g. communication is done over the internet), the choice is oftentimes narrowed down to AP or CP. Specifically, in the case of network partitioning, a choice must be made regarding to provide either availability or consistency.

%Consensus mechanisms used within blockchain systems must adhere to the CAP theorem \citep{RN47}. In particular, in the case of network partitioning, the system must either make compromises towards consistency or availability. Examples of this can be seen in systems utilizing Nakamoto style consensus, in which forks may happen, creating periods of inconsistency within the network. The system therefore sacrifices strong consistency in favor of availability. In contrast to this, systems using deterministic BFT style consensus algorithms cannot fork, and such opt for strong consistency, sacrificing availability in the event of network partitioning. 

%This can further be related to a consensus algorithm's transaction finality; the algorithm's guarantee that committed transactions cannot be reversed. Consensus algorithms providing probabilistic finality, e.g. Nakamoto style consensus, favor availability over strong consistency. Consensus algorithms providing immediate finality, e.g. BFT style consensus, need strong consistency to enforce this, thus sacrificing the system's availability during network partitioning.     

\subsubsection{FLP Impossibility}
\label{subsub:FLP}

% result

An important result within distributive systems is the so called \textit{FLP Impossibility} result. \citet*{RN40} prove that one cannot achieve deterministic consensus in an asynchronous, distributed system with at least a faulty node. This has major implications on consensus in blockchain systems, as communication between peers are over the internet in most practical settings, which is inherently asynchronous, and one oftentimes desire some non-zero level of fault tolerance. 

\citet{RN40} reach this conclusion by proving that in the fully asynchronous setting, utilizing a deterministic consensus algorithm, there exist some configuration of nodes $C$, in which the system cannot reach an decision, given at least a faulty node. In specific, given a network of N nodes, all with some input value $x_i \in \{0,1\}$, with the goal of agreeing upon a common output value $y \in \{0,1\}$, there exist a configuration of input values among the nodes in which $y$ may be undecided\footnote{\citet{RN40} scenario is specifically related to that of Binary Byzantine Agreement, but can be extended to consensus about non-binary values. }. 

The authors prove this by making the observation that there must exist two configurations $C_0$ and $C_1$ which lead the consensus algorithm to agree on different values, but which also only differ in the input value of a single node $n$. Such, the result of the consensus round depends on the value contributed by the node $n$. Without loss of generality, assume that $C_0$ gives an output $y = 0$ and $C_1$ gives an output of $y = 1$.  Should $n$ be faulty (i.e. it does not contribute its value during the consensus round), $C_0$ or $C_1$ cannot be differentiated, and thus should decide upon the same value, as the consensus algorithm is deterministic. If the value they decide upon is $y = 1$, then $C_0$ is indecisive; the configuration may lead to either values being decided upon. The same holds for $C_1$ in the case of $y = 0$. Therefore, there exist some configuration $C$ in which one cannot deterministically decide upon a value.

The authors go on to show that there exist some schedule $\sigma$ of events, which from an indecisive configuration $C$, lead to a continuous cycle of going from indecisive configuration to indecisive configuration. Specifically, the authors show that by sufficiently delaying some event $e$, there always exist a transition from one indecisive configuration to another. Thus, there exist some schedule $\sigma$ where the system cannot decide upon any values and can therefore not reach any forward progress; the consensus algorithm does not have liveness. 

% talk about the result and what it shows


In search for practical consensus mechanisms, major work has been directed towards consensus algorithm which can circumvent this result \citep{RN46, PBFT_MIT, RN51, RN42}. Specifically, the FLP impossibility holds for the scenario of a deterministic consensus algorithm, providing both safety and liveness, in a fully asynchronous network with at least a single faulty nodes. Such, by removing any of these assumptions, the result do not hold. In practical settings however, safety, liveness, as well as fault tolerance are oftentimes seen as mandatory. Therefore, the only way to circumvent the results are related to altering the synchronicity assumption about the network or the determinism of the consensus algorithm. In particular, consensus models which are non-deterministic, i.e. introduce randomization, do not adhere to the result \citep{RN51}. 


\subsubsection{Synchrony, Partial Synchrony and Asynchrony}

Additionally, in order to avoid the impossibility result \citep{RN40}, one can make the assumption that the underlying communication network is synchronous; messages between peers are delivered within some known fixed upper bound $\Delta$. This oftentimes do not reflect reality however, as communication over the internet is susceptible to delays and network failure. Thus, synchrony may not be enforceable in practical systems, depending on the characteristics of the network.

\citet{RN46} introduce the aspect of a partially synchronous network. It creates a middleground between synchronous and asynchronous networks, in which the upper bound $\Delta$ do exist, but it may either be not known a priori or may not hold before a certain point of time (i.e. eventually synchronous). This is sufficient to circumvent the FLP impossibility result. It however poses challenges related to the design of consensus mechanisms; if the bound cannot be known a priori, the consensus algorithm must be able to function regardless of what actual value the bound takes. If the bound only holds eventually, after some point of time $T$, the consensus algorithm must be able to function before $T$. 

As mentioned in section \ref{subsub:FLP}, the FLP impossibility result only hold for deterministic consensus. Thus, randomized consensus models may still achieve consensus in asynchronous network, assuming no upper bound $\Delta$ on the message delay between peers in the network. 

Based of this, the timing assumptions made by a consensus algorithms can be categorized accordingly:

\textbf{Synchronous:} There exist a known fixed upper bound $\Delta$ on the message delay between peers within the network.

\textbf{Partial Synchronous:} Either of the following statements hold: \begin{enumerate}[i]

    \item There exist a upper bound $\Delta$ on the message delay between peers within the network, but it cannot be known a priori.
    \item There exist a upper bound $\Delta$ on the message delay between peers within the network, but it does not hold before an unknown point of time $T$.
\end{enumerate}

\textbf{Asynchronous}: There does not exist a known fixed upper bound $\Delta$ on the message delay between peers within the network.


\subsection{Security considerations in blockchain systems}

\label{subsec:security}



When designing a blockchain system, there are several security aspects to considers. \citet{RN17} and \citet{RN30} provide insight into some core security issues related to blockchain systems. This section describes several of the most central security considerations towards blockchain systems, based on their reviews.

The concept of \textit{consistency} in relation to a blockchain system refers to its ability to keep the ledger consistent across the participants of the network \citep{RN17}. As stated by the CAP theorem \citep{CAP}, a distributed system cannot guarantee strong consistency, availability and partition tolerance simultaneously. Blockchain systems may therefore utilize different approaches in terms of consistency. In particular, common approaches implemented by  blockchain system are strong consistency, ensuring that nodes keep the same ledger at all times, and eventual consistency, in which nodes may have differing ledgers at some specific point of time, but eventually become consistent. Here, strong consistency comes with the trade-off of reduced availability in the event of network partitioning, while eventual consistency introduce the need for conflict resolution, should there be a dispute regarding which ledger is correct. 

\textit{Tamper-Resistance}, in terms of a blockchain system, refers to the system's ability to ensure the integrity of the information stored in its ledger, during and after block generation \citep{RN17}. Specifically, when new blocks are propagated within the system, the system's nodes need to be able to assert the validity of the transactions contained within the block. Adversaries may in particular attempt to modify a transaction to be included in the new block, or transactions already part of the ledger. Both are conventionally avoided by the use of strong cryptographic mechanisms, utilizing secure hash functions to assess that the integrity of transactions and blocks are not compromised, as well as digital signatures, ensuring that the transaction's origin are who they claim to be. 


Essential to system is its requirements towards \textit{Byzantine Fault Tolerance}. In a trustless peer-to-peer network, some degree of Byzantine fault tolerance is needed, to protect against arbitrary or malicious behavior by network participants.  The degree may then again vary depending on the setting of the system, whether it is permissioned or permissionless. Commonly labeled as the \textit{51\% attack}, malicious actors have been conjectured to have the ability to override honest transactions in cryptocurrencies like Bitcoin or Ethereum, given a majority of the hashing power of the network. This is further applicable to traditional BFT consensus models, where the system commonly assumes a maximum number of faulty nodes $f$, providing implications on the total number nodes required for consensus, and thus the scalability of the model.  

Another common attack vector within P2P systems is the \textit{Sybil attack}, where malicious actors create multiple fake identities, attempting to increase their influence upon the network. This is elegantly addressed in Nakamoto's Proof-of-Work scheme \cite{Nakamoto_Bitcoin_POW}, linking voting power to hashing power, thus making Sybil attacks ineffective. It is also addressed in permissioned blockchain systems, requiring all participants of the network to be authenticated, linking each identity to real world entities. The attack is consequently especially relevant in permissionless settings. 

Related to cryptocurrencies like Bitcoin, there is the \textit{Double spend attack}. This specifically refers to the action of spending a single amount of currency twice, i.e. in two separate transactions. In Bitcoin, this is partially dealt with by ensuring the integrity of transactions and including digital signatures, ensuring that parties partaking in the transaction are who they claim to be. Furthermore, transactions are only assumed to be confirmed after $k$ succeeding blocks, making the chance of reversing a previously committed transaction small. However, since the system's consensus termination is probabilistic, the potential for a fork is still there, enabling a double spend attack. This is further highlighted through the \textit{Blockchain Anomaly} \citep{RN38}, showing the impossibility of guaranteeing that certain committed transactions will not be removed from the main chain in the future. 

% start at early point of blockchain. build blocks privately, can forge time stamps to allow quicker generation of blocks. Publish larger chain later, causing double spends.
Some blockchain systems may also be vulnerable to a \textit{Long-Range attack} \citep{RN55}. Related to other majority consensus attacks, instead of attempting to hijack $k$ block confirmation limit, the attacker forks the chain at a much earlier point. The alternative chain is then privately mined upon by the attacker. \citet{RN55} proposes that in some types of blockchain systems, e.g. earlier versions of the Ethereum client, the attacker can take advantage of the fact that they are the only entity contributing to the alternative chain, accelerating the rate in which blocks are generated. This can then be used to overtake the main chain, enabling double spend attacks. \citet{RN55} goes on to explain that blockchain systems may protect against such attacks by limiting the variability among alternative chains. 

Another possible attack, the \textit{P+ Epsilon attack}  \citep{RN54}, leverages non-altruistic participants in the attacker's favor. By promising to provide some kind of reward, denoted $\epsilon$, the attacker can align other participants' incentives according to their own, creating a dominant strategy within the network. This then allows the attacker to carry out their goals, despite not controlling a majority of the network themselves, assuming that altruists do not constitute a majority within the network. The attacker may later on not pay out the reward promised, reaping the profit of the attack all by themselves \citep{RN30}.  

The \textit{balance attack} constitutes another flavor of the double spend attack, allowing malicious actors to force double spend attacks despite an honest majority, given sufficient network delay. \citet{RN39} provide a theoretical analysis of the attack and demonstrate its feasibility through experimental results, utilizing the Corda blockchain platform. The attack provides a valid security concern regarding use of proof-of-work based consensus schemes in blockchain systems with considerable network delay. 

\textit{Border Gateways Protocol Hijacking} (BGP) involve an attacker taking control over parts of the Internet routing infrastructure utilized by the blockchain system \citep{RN53}. By controlling key parts of the routing mechanisms of the network, attacker may be able to both partition the network, isolating participants from communicating with their peers, as well as significantly delaying block propagation. \citet{RN53} goes on to demonstrate the feasibility of both types of attacks. Similar to that of a balance attack, this can be used to perform double spends in certain types of blockchain systems. 

Blockchain systems may also be susceptible towards \textit{distributed denial of service} (DDOS) attacks. In particular, if the consensus model is leader-based, the system's liveness may be threatened. By overloading the leader with incoming traffic, this may prevent them from carrying out the consensus algorithm and thus impact the transaction throughput of the system. Furthermore, DDOS attacks may have implications on the number of faulty nodes of the system. This may impact the consensus scheme directly, in the case of BFT algorithms. It may also impact it indirectly, by altering the distribution of available computational resources, shifting the balance of power in the case of Proof-of-Work based consensus algorithms. 

To conclude, the \textit{degree of centralization} of a blockchain system may impact its security. Within certain consensus models, centralizing power within a subset of the nodes have inherent risks. It may provide incentive for DDOS attacks, as powerful nodes have greater influence upon the network, thus increasing the impact of an attack. It may furthermore heighten the risk of collusion, reducing the number of nodes for an adversary to corrupt. This may then lead to potential abuse of power, in form of double spend attacks.

Additionally, \citet{RN17} propose the security properties of \textit{user anonymity}, \textit{transaction confidentiality} and\textit{transaction unlinkability}. These properties all relate to the privacy of participants partaking in the blockchain system, protecting their identity and the confidentiality of the data they commit to the blockchain. This may be of great benefit in the setting of financial system, e.g. a cryptocurrency like Bitcoin, in which lack of privacy may enable attacks against lucrative targets. In an authenticated setting, it may be less applicable. 

\autoref{tab:background_security_considerations} provides a brief summary of the security considerations discussed. In terms of the SCM setting, with a permissioned blockchain system affected by limited network throughput, Byzantine fault tolerance, BGP and DDOS susceptibility are deemed the most generally applicable security considerations. Given that participants in the system are authenticated, a Sybil attack can effectively be combated. Furthermore, in the case of immediate transaction finality, which is provided by several types of consensus algorithms, forking is not possible. Thus,  long-range, P+ epsilon and balance attacks are therefore only applicable to Nakamoto style consensus algorithms, having probabilistic transaction finality. Finally, considering an authenticated setting, aspects like user anonymity and transaction unlinkability are deemed not relevant, while transaction confidentiality may be desired. 


\todo{Remove this table, or extend the table to substitute the section}

\renewcommand{\arraystretch}{1.25}
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm}p{7cm}}
         Name & Description \\\hline
         Consistency & Which approach will the system utilize to ensure the consistency of the system's ledger?  \\
         Tamper-Resistance & Is the system able to ensure the integrity of the ledger? \\
         Byzantine Fault Tolerance & To which an extent do the system need to tolerate Byzantine faults, e.g. adversarial nodes?  \\
         Sybil attack & How will the system protect against malicious actors creating multiple fake identities, attempting to outvote an honest majority?  \\
         Double spend attack & How will the system prevent nodes spending the same currency for two separate transactions? Specifically related to cryptocurrency systems.  \\
         Long-Range attack & To which extent is the system vulnerable to Long-Range attacks; forking the blockchain at its genesis block and privately building an alternative chain?  \\
         P+ Epsilon attack & To which extent is the system vulnerable to P+ Epsilon attacks; taking advantage of the dominant strategy among network participants, leveraging non-altruistic participants against the system? \\
         Balance attack & To which an extent is the system vulnerable to balancing attacks; splitting the network into sub-networks, delaying transactions and performing double spend attacks? \\
         Border Gateways Protocol \hspace{0.5cm} Hijacking & How will the system handle adversarial attacks against the network's routing mechanisms; partitioning the network or delaying block propagation? \\
         DDOS susceptibility &  To which an extent is the system susceptible to DDOS attacks, in terms of impact upon safety and liveness? Especially relevant for leader based consensus models. \\ 
         Degree of centralization & To which an extent is the system centralized around a subset of participants? This may have implications on various double spend attacks, as well as DDOS susceptibility.   \\
         User anonymity & Are participants of the system able to partake in transactions while staying anonymous?\\
         Transaction confidentiality & To which extent are transactions kept confidential? \\
         Transaction unlinkability & To which extent is it possible to link a group of transactions to a specific identity?\\
    \end{tabular}
    \caption{Security considerations for blockchain systems}
    \label{tab:background_security_considerations}
\end{table}

==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/conclusion.tex <==
\section{Conclusion and Future Work}

The purpose of this study is to analyze how the state of the art consensus algorithms relate to SCM blockchain systems in an enterprise setting with multiple stakeholders, affected by limited network throughput and poor network quality.  The mapping study's classification emphasizes how well the consensus algorithms can satisfy performance, integrity, and security requirements in a degraded network environment. The study gives insights into the advantages and weaknesses of the investigated consensus algorithms. Our future work will evaluate and compare the consensus algorithms identified from this study more quantitatively by running simulations and experiments.

\begin{comment}

This section provides a summary of the paper; related work, its motivation and main contributions. Furthermore, it elaborates on the limitations of the research, as well as considerations for future work.

\subsection{Summary of related work}

In recent years, there has been conducted vast amounts of research in the domain of blockchain technology. Especially, larger focus has been dedicated to presenting state of the art consensus algorithms, current project initiatives and the potential use cases blockchain technology has in certain domains. Particular interest has been dedicated to the usage of blockchain technology within financial services. Usage within supply chain management, while highlighted as a promising domain, has nonetheless seen less contribution. There currently exists little research related to solving some of the major challenges the domain faces; tracking of supply goods, over a larger geographical area, despite limited throughput within the network. 

\subsection{Research motivation}

In the search of unlocking the full potential of utilizing blockchain technology within supply chain management, there is a clear need for creating adequate blockchain platforms. Part of the solution will be the selection of core consensus mechanisms. The goal of this research project is to provide insight into core mechanisms of state of the art consensus algorithms, and how they relate to SCM blockchain systems, in an enterprise setting with multiple stakeholders, affected by varying network throughput. As related work has largely focused on applications within financial services, this project may provide insight into novel challenges related to consensus in SCM blockchain systems. 

\subsection{Contributions}

This paper presents a novel systematic mapping study, surveying both state of the art and novel consensus algorithms for use within the blockchain ecosystem, in terms of usage within enterprise, permissioned blockchain systems affected by limited network throughput. The mapping study's classification emphasizes the consensus algorithms communication related costs and the timing assumptions they make regarding the underlying network.

\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}

It is deemed that limited network throughput may cause increased asynchrony within a blockchain system; it is not feasible to make assumptions regarding the ordering or timing messages being sent. Synchronization assumptions made by consensus algorithms may therefore be hard to adhere to. In particular, consensus algorithms which assume a synchronous network, in the form of known upper bound on the message delay $\Delta$, cannot provide integrity in this environment. Specifically, it is deemed that Nakamoto style consensus algorithms are unfit for the relevant application scenario. 

Furthermore, it is also noted that while consensus algorithms assuming a partial synchronous network provide integrity, even in periods of asynchrony, they cannot provide forward progress at the same time, hampering transaction throughput. Because of this, consensus algorithms assuming an asynchronous network may be especially relevant, providing more stable transaction processing, while avoiding having to tune configuration parameters related to network latency. 

\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput?}

Given the aforementioned asynchronicity of the network, consensus algorithms relying on a synchronous network for security reasons are unfit for usage in the relevant setting. In particular, Nakamoto style consensus algorithms may be subject to double spend and balance attacks, given sufficient network delay, even in the case of an adversary with very limited control of the network. 

Further, it is deemed that in blockchain systems with limited network throughput, DDOS attacks are increasingly relevant in a network affected by poor network throughput. In particular, leader-centered consensus models may be exploited, as adversaries overwhelming them with incoming traffic will hinder the system's liveness. This is specifically relevant to BFT, Hybrid and Crash tolerant consensus algorithms. Additionally, a similar attack can be executed in the context of Federated Byzantine Agreement consensus algorithms, were well-connected nodes are targeted by a DDOS attack, creating divergence within the network.

Another type of attack, Border Gateway Protocol Hijacking, is deemed generally applicable against most consensus algorithms, in that partitioning the network and sufficiently delaying communication among nodes is enough to halt the algorithm's liveness, and in extreme cases, its safety guarantees. In an environment which is affected by limited network throughput, these types of attacks would be more practical, given lower throughput of network packets to manipulate throughout the network. 



\subsection{Future work}

To provide further insight into the performance characteristics of consensus algorithms in low network throughput blockchain systems, experimental studies are warranted. By implementing candidate consensus algorithms for relevant blockchain platforms, a more detailed comparison can be given, especially in terms of performance under relevant network scenarios and security attacks. In particular, it could be deemed interesting to look at comparative data as to what performance gain an asynchronous consensus algorithm like HoneyBadgerBFT would provide over a partially synchronous consensus algorithm like PBFT, given varying network throughput.

Furthermore, it is also deemed interesting to look at the degree in which poor network throughput has on the asynchronicity of the network, varying the number of nodes affected by it. There might also be certain implementation specific optimizations which can be introduced, which can allow a system to more effectively deal with the limited network throughput.



























%A limited network throughput may also cause increased asynchrony. Synchronization assumptions made by consensus algorithms may therefore be hard to adhere to. Because of this, asynchronous protocols may be especially relevant, providing a better fit for the network model, while avoiding having to tune parameters related to network latency. 

%Based of a systematic mapping study, the following consensus paradigms were identified: Nakamoto, Byzantine Fault Tolerant, Federated Byzantine Agreement, Hybrid and Crash Tolerant consensus algorithms.

%Nakamoto style consensus provide strong performance characteristics in terms of communication cost. However, in an authenticated, enterprise setting the lottery mechanisms native to the consensus algorithms may have to great an impact on transaction throughput, especially if deterministic finality is also desired.

%BFT style consensus provide high transaction throughput, but may suffer from poor scalability, given quadratic communication complexity. New developments related to algorithms with linear communication complexity may solve this problem, making a good case for usage within SCM. In an authenticated, permissioned setting, these new innovations may be deemed the best alternative, given an stable, agreed-upon network structure. 

%Federated Byzantine agreement algorithms decentralize the trust structure of the network, but it is unclear if this is needed in an enterprise SCM setting. The algorithms furthermore provide no guarantees towards consensus latency, and such may not perform well in a network characterized by low network throughput.

%Hybrid consensus approaches bridge the gap between Nakamoto and BFT style consensus, and provide a separation between leader election and transaction verification. This is especially relevant to the permissionless setting, where Sybil attack resistance is essential. In an enterprise SCM setting, with a permissioned network, this may be superfluous. If a BFT style consensus scheme is sufficient, i.e. Sybil attack resistance is not needed, the Nakamoto part of the hybrid approach may be an unneeded computational cost. 

%Crash tolerant consensus algorithms provide great performance characteristics, but are only applicable to private blockchain systems. Furthermore, there are concerns related to its applicability to a network affected by low network throughput, given strong synchronization assumptions and a leader-centered structure. 

\end{comment}

==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/cover.tex <==
\title{Consensus in Blockchain Systems with Low Network Throughput: A Systematic Mapping Study\\
%{\footnotesize \textsuperscript{*}Note: Sub-titles are not captured in Xplore and should not be used}
%\thanks{Identify applicable funding agency here. If none, delete this.}
}

\author{\IEEEauthorblockN{1\textsuperscript{st} Henrik Knudsen}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{Norwegian University of Science and Technology}\\
Trondheim, Norway \\
henriknu@stud.ntnu.no}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Jakob Svennevik Notland}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{Norwegian University of Science and Technology}\\
Trondheim, Norway \\
jakob.notland@ntnu.no}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Peter Halland Haro}
\IEEEauthorblockA{\textit{Sintef Nord AS} \\
\textit{Sintef Nord}\\
Tromsø, Norway \\
peter.haro@sintef.no}
\and
\IEEEauthorblockN{4\textsuperscript{th} Truls Bakkejord Ræder}
\IEEEauthorblockA{\textit{Sintef Nord AS} \\
\textit{Sintef Nord}\\
Tromsø, Norway \\
truls.rader@sintef.no}
\and
\IEEEauthorblockN{5\textsuperscript{th} Jingyue Li}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{Norwegian University of Science and Technology}\\
Trondheim, Norway \\
jingyue.li@ntnu.no}
}

\maketitle

\begin{abstract}
%Blockchain is an emerging technology, tracing back to the rise of Bitcoin and other cryptocurrencies. Recent years have seen its adoption in other promising domains, in particular, supply chain management. While there currently exist platforms offering tools for developing enterprise blockchain solutions for SCM, they have low maturity and are not capable of supporting core business goals; The tracing and delivery of goods over  large  geographical  areas,  involving  numerous  stakeholders  and  governance  sectors. As part of the initiative of facilitating adequate platforms, this specialization project aims to identify core consensus mechanisms which both can provide integrity, as well as security for SCM blockchain systems affected by varying throughput. Through a systematic mapping study, current state of the art and novel consensus algorithms are classified, with particular focus on their communication costs and timing assumptions made about the network. The following analysis deem that consensus algorithms relying on a synchronous network for correctness cannot provide integrity in the relevant setting. Furthermore, consensus algorithms may be particular susceptible towards distributed denial of service and routing attacks, given limited network throughput. Conversely, asynchronous consensus algorithms are deemed robust towards many of these attacks, and may furthermore provide high transaction throughput in events of asynchrony. Based on this, asynchronous consensus algorithms are deemed promising in the setting of blockchain systems affected by varying network throughput.%
%Blockchain as an emerging technology provided disruption within multiple domains by delivering novel distributed peer-to-peer networks solving the double spend problem without a trusted third part as originally defined by Nakamoto\cite{Nakamoto_Bitcoin_POW}. The technology has matured significantly, spawning a whole new field defined as distributed ledger technology\cite{ davidson2016disrupting} which has been adopted to multiple fields, particularly in supply chain management (SCM). Multiple frameworks have been designed for developing enterprise blockchain applications for SCM, however, they are insufficient for tracking and delivering perishable goods across large geographical areas, across multiple sectors and stakeholders. Removing the inevitable visibility shortage in the supply chains and integrating data internet of things (IOT) devices collated with other data in the supply chain across varying network quality are still active research topics, thus the existing frameworks are incapable of supporting the core business goals. 
Blockchain technologies originate from cryptocurrencies. Thus, most blockchain technologies assume an environment with a fast and stable network. However, in some blockchain-based systems, e.g., supply chain management (SCM) systems, some Internet of Things (IOT) nodes can only rely on the low-quality network sometimes to achieve consensus. Thus, it is critical to understand the applicability of existing consensus algorithms in such environments. We performed a systematic mapping study to evaluate and compare existing consensus mechanisms' capability to provide integrity and security with varying network properties. Our study identified 25 state-of-the-art consensus algorithms from published and preprint literature. We categorized and compared the consensus algorithms qualitatively based on established performance and integrity metrics and well-known blockchain security issues. Results show that consensus algorithms rely on the synchronous network for correctness cannot provide the expected integrity. Such consensus algorithms may also be vulnerable to distributed-denial-of-service (DDOS) and routing attacks, given limited network throughput. Conversely, asynchronous consensus algorithms, e.g., Honey-BadgerBFT, are deemed more robust against many of these attacks and may provide high integrity in asynchrony events.

\end{abstract}

\begin{IEEEkeywords}
Blockchain, consensus, security, integrity, performance and supply chain
\end{IEEEkeywords}

==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/discussion.tex <==
\section{Discussions}

\subsection{Comparison with related work}

Numerous surveys, e.g., \citep{RN21, RN18, RN22, RN17} have been dedicated to present and classify consensus algorithms according to their performance characteristics. In particular, \citep{RN21} and \citep{RN18} present novel evaluation frameworks for analyzing consensus algorithms. \citep{RN21} furthermore highlights the impact network synchrony has on consensus algorithms. Our study differs from related work because it focuses on consensus algorithms' performance characteristics in the specific application scenario in which the network is constrained by varying network throughput. Furthermore, our classification scheme is skewed towards the impact of communication costs and timing assumptions on the algorithms' performance, utilizing the metrics of communication latency, communication complexity, and timing assumptions.

Studies \cite{RN17, RN30, RN21} focuses on the security properties of consensus algorithms, including that of ensuring the integrity of the blockchain. \citep{RN17} discusses core security properties of consensus algorithms and their ability to ensure consistency and tamper-resistance across a blockchain system's ledgers. \citep{RN30} furthermore discusses the circumstances in which these properties may be broken. \citep{RN21} discusses how consensus algorithms may function in a fully asynchronous setting. Our study differentiates from \cite{RN17, RN30, RN21} in that it investigates how consensus algorithms ensure integrity in the specific application scenario in which the network is constrained by varying network throughput. The scenario includes both increased asynchrony of the network, as well as isolation of nodes. It thus provides a unique perspective into which consensus algorithms can provide safety and integrity in such a constrained environment.

%Several studies identified have focused on the security aspect of consensus algorithms used within blockchain systems \citep{RN17, RN30}. \citet{RN17} proposes essential security properties of blockchain systems, including its resistance towards DDOS and double spend attacks. Reference \citet{RN30} provide further insight into security threats towards blockchain systems, including Long-Range, P + epsilon and Border Gateway Protocol Hijacking attacks. This research stands out among related work in that it investigates how consensus algorithms ensure security in the specific application scenario in which the network is constrained by varying network throughput. The scenario includes both increased asynchrony of the network, as well as isolation of nodes, and thus provides a unique perspective into what security threats may be especially relevant in such a constrained environment. Compared to the related work \citep{RN17, RN30}, this research also provide a broader overview, including a total of 25 consensus algorithms in the analysis. 


\subsection{Known limitations}

This study does not provide insight into experimental data for the different consensus algorithms surveyed. It is, therefore, difficult to draw comparisons regarding transaction throughput among different categories of consensus algorithms.

Furthermore, this study focuses on consensus in enterprise and permissioned blockchain systems affected by limited network throughput. Blockchain systems that do not fit a similar application scenario may emphasize other factors rather than those presented by our classification scheme. The security aspect of this study is based on the reviews of \citep{RN17} and \citep{RN30}. While it is deemed that these works constitute a comprehensive review of security attacks generally applicable to blockchain systems, there may be other security attacks to consider, given the specifics of the blockchain system in question or the scenario in which it is utilized.



\begin{comment}


\begin{table}[h]
    \centering
    \begin{tabular}{lp{10cm}}
          \multicolumn{2}{p{\textwidth}}{\textbf{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}}\\\hline
          
          Nakamato consensus & Unable. Rely on network synchronicity for integrity. \\
          Byzantine fault tolerant & Able, for majority. Linear-BFT may struggle, because of synchronicity assumptions.   \\
          Federated Byzantine Agreement & Able. \\
          Hybrid & Able. \\
          Crash tolerant & Able. \\
          \multicolumn{2}{p{\textwidth}}{\rule{0pt}{6ex}\textbf{RQ2: What consensus models are able to provide security in an environment with limited network throughput?}}\\\hline
          Nakamato consensus & Unable. Lack of network synchronicity may allow for double spend and balance attacks. \\
          Byzantine fault tolerant & Able. However, consensus algorithms are susceptible to DDOS attack towards leader, hurting liveness. HoneybadgerBFT is not affected by this. \\
          Federated Byzantine Agreement & Able. However, well-connected nodes may be susceptible to DDOS attack, hurting liveness. \\
          Hybrid & Able. However, consensus algorithms are susceptible to DDOS attack towards leader, similar to BFT. \\
          Crash tolerant & Able. However, consensus algorithms are susceptible to DDOS attack towards leader, similar to BFT. \\
    \end{tabular}
    \caption{Summary of how surveyed consensus algorithms relate to RQ1 and RQ2.}
\end{table}

\end{comment}


%\subsection{Nakamoto Consensus}


% In terms of classification, they score well according to the classification. 
%Nakamoto Consensus style consensus algorithms commonly provide consensus in a single communication step, with linear communication complexity. Additionally, the consensus algorithms provide optimal Byzantine Fault Tolerance, only requiring an honest majority. 

%\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}
% Separate probabilistic finality from paragraph, comment Casper the finality gadget and other overlay on top of POW, giving deterministic finality

%The consensus algorithms have probabilistic finality, oftentimes following the longest chain rule to solve fork disputes. This may be problematic, as this opens up for double spend and balance attacks, should there be sufficiently high delay among the network's nodes. Developments have been made in order to mitigate this. In particular, finality gadgets like Casper have been proposed \citep{RN43}, which can overlay proof of work blockchain systems, providing deterministic finality.  

%In terms of the classification, the group perform impressively. While probabilistic finality is not ideal, Nakamoto style consensus algorithms provide optimal communication complexity, few communication steps and high Byzantine Fault Tolerance. One might however argue that it is not a fair comparison, as while BFT style consensus algorithms' bottleneck is oftentimes related to communication costs, Nakamoto style consensus algorithms have other aspects which affect transaction throughput. As an example, in the original consensus scheme proposed by Nakamoto \citep{Nakamoto_Bitcoin_POW}, transaction throughput is directly linked to the security of the system; in order to increase transaction throughput, the global block timer must be lowered, making forks more likely and reducing security. 

%In terms of the SCM setting, with nodes distributed over a large geographical area and with potentially high network latency, PoET stands out among the Nakamoto style consensus algorithms in that it would be significantly affected. As the algorithm internally uses a random wait timer to determine leader election, it must adhere to this increased latency, and thus increase the wait timer as well, to ensure fairness.   

%\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput? }


%Related to security, Nakamoto style consensus algorithms have low susceptibility to DDOS attacks. In contrast to many other types of consensus schemes, which are centered around a stable leader, Nakamoto style consensus algorithms elect leaders non-deterministically on a block-to-block basis. This makes DDOS attacks infeasible in practical settings. 

%A major security concern regarding the consensus algorithms is related to their synchronization assumptions regarding the network. While the original Bitcoin proof of work scheme has proven security in a synchronous network model \citep{RN44}, the protocol cannot provide integrity or security in a fully asynchronous setting \citep{RN45}. In particular, given sufficient long communication delay among nodes, the system can be exploited, even if the adversary only control a fraction of the computational power of the network. Given an environment characterized by varying network throughput and asynchrony, this is obviously problematic.


%\subsection{Byzantine Fault Tolerant}

%Byzantine fault tolerant algorithms commonly provide consensus in a three communication step process, with quadratic communication complexity. Some algorithms found in this paper, namely Delegated BFT, Mixed BFT and Linear-BFT, achieve linear communication complexity, through partitioning the network. In particular, Delegated BFT and Mixed BFT delegate consensus to a subset of the nodes in the network, while Linear-BFT reduce the amount of messages sent per node by using an expander graph. This, however, comes at a cost of either significantly increased centralization or potentially higher consensus latency.

%\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}

%BFT style consensus algorithms all provide deterministic finality, which may be of major benefit, providing low confirmation latency for transactions. In the enterprise setting, this can be deemed a differentiating factor, providing greater flexibility in business operations. 

%The consensus algorithms generally can withstand a maximum of a $\frac{1}{3}$ Byzantine nodes, posing a significantly weaker resistance than the honest majority threshold provided by Nakamoto style consensus algorithms. Linear-BFT emerges as a promising innovation, providing the optimal threshold of $\frac{1}{2}$ Byzantine nodes, while also having amortized optimal communication complexity of $\Theta(n)$. This is accomplished by the use of a threshold signature scheme \citep{RN41} and an expander graph, removing the need for quadratic all-to-all communication to achieve consensus.


% Security considerations
% Decentralization problems, especially relevant for Delegated BFT and 

% Consensus algorithms make claims that the system is synchronous. Problematic in terms of systems with high degree of a asynchrony
%Related to the SCM setting, nodes may be distributed over a large geographical area and such may experience high communication latency. This may be problematic for a large portion of BFT style consensus algorithms, as they make underlying assumptions as to the synchrony of the network. In particular, many of the algorithms assume a known upper-bound on the message delay $\Delta$. This may be used to organize communication within the network, and to determine whether a node is unresponsive. Given the large potential distance between nodes, this upper bound may be larger than desired, negatively impacting transaction throughput.

%Furthermore, in terms of nodes experiencing low network throughput and poor connection, this may pose a serious problem related to the synchrony of the network. It is infeasible to increase the message delay $\Delta$ to accommodate this, as this would have to great an impact on transaction throughput. Treating such network failures and times of asynchrony as an extreme case, and keeping the message delay $\Delta$ relatively low, these nodes would be deemed faulty in such events. This of course effectively reduces the fault tolerance of the network, as the remaining nodes of the network cannot distinguish the network failure from a Byzantine fault. Once normal operation is started anew, these nodes must be brought up to speed. An interesting direction to pursue would be looking at potential optimizations to implement, in terms of checkpoint management, state transfer and view change protocols, to handle such such events in an as performant way as possible.

%In light of this, the HoneyBadgerBFT consensus algorithm differentiates itself, as it makes no assumptions regarding the synchrony of the network. Functioning purely asynchronously, it may avoid the performance impact of a larger message delay $\Delta$. In particular, \citet{RN42} points out that there will always be a inherent trade-off related to such synchrony assumptions. If the $\Delta$ parameter is too low, the system will not provide progress; if too high, it will not be able to fully take advantage of the network's bandwidth. The authors go on to propose HoneyBadgerBFT as a candidate for consortium blockchain systems, emphasizing its benefits of robustness and high transaction throughput, despite an asynchronous system. 



%\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput? }
% DDOS susceptibility

%In terms of security, BFT style consensus algorithms have an increased susceptibility towards DDOS attacks, compared to Nakamoto style consensus. Specifically, should a sufficiently powerful adversary have insight into which of the network's nodes is the leader for a given election term or view, they could impare the system's liveness by overloading the leader with incoming traffic. This is exasperated in the relevant setting, of low network throughput. As many BFT style consensus algorithms rely on a stable leader for progress, in the worst case, this could lead to a continuous view change, grinding transaction throughput to a halt. 





%\subsection{Federated Byzantine Agreement}


%Federated Byzantine Agreement consensus algorithms, like RPCA and SCP, do not provide any guarantees as to the number of consensus steps involved in agreeing upon a set of transactions. As nodes only communicate within their respective quorum slice, communication complexity depends on the size of each node's quorum slice. In Ripple, UNL lists need to overlap 90 \% across the network to ensure security, which makes communication complexity $\Theta(n^2)$. In SCP, nodes are free to pick their own quorum slices, based on their own reasoning (e.g. reputation, wealth, brand). In an optimistic setting, where the size of quorum slices are constant, this makes SCP's communication complexity $\Theta(n)$. 

%\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}

%Both RPCA and SCP make synchronization assumptions related to the underlying network; they both provide safety in periods of asynchrony, but require messages to at some time be bounded by some known upper bound message delay $\Delta$ to provide liveness. SCP provide optimal resilience towards Byzantine nodes in the federated setting, only requiring that nodes' quorum slices intersect honestly, while RPCA makes an assumption of maximum 20 \% Byzantine nodes for a given UNL list. 

%The major benefit of RPCA and SCP are that they provide byzantine agreement in a decentralized fashion; there is no need for a central authority or initial consensus among participants to establish which nodes are to be part of the network. In practice, this is questionable in terms of RPCA, given the significant requirement towards UNL overlap of 90\%, leaving nodes with little choice as to what nodes they want to trust. SCP provide greater options in this aspect. 

%To which degree this is beneficial in the SCM setting is unclear. If there is broad agreement among stakeholders towards what organizations are to constitute the network, then this flexibility is too little benefit. In fact, BFT style consensus algorithms would perform better in this case. However, in the case in which there is no such overarching agreement, federated byzantine agreement may allow for cooperation among organization which would otherwise never occur.  

%Another aspect to consider is the effect of low network throughput on federated byzantine agreement. As federated byzantine agreement builds upon nodes' quorum slices intersecting, consensus relies on that not all these interconnections become faulty. Should these important nodes suffer from low network throughput, this could hamper the speed and throughput in which transactions can be processed by the network. In particular, if they are unable to respond for a longer period of time, transaction throughput may halt. Combined with the lack of guarantees in terms of consensus latency, as well as the need for synchrony to guarantee liveness, it is questionable whether federated byzantine agreement would perform well in such a network. 


%\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput? }

%In terms of security, federated byzantine agreement avoids some of the pitfalls related to BFT style consensus. In particular, as RPCA and SCP are leaderless consensus algorithms, there is no vulnerability related to a leader being targeted by a DDOS attack, stopping the system from achieving progress.

%There is however a new potential attack vector, related to a \textit{divergence attack}. Going back to the important role in which intersecting nodes play in federated Byzantine agreement, a worrisome attack a sufficiently powerful adversary could perform is a  DDOS attack targeting intersecting nodes. This has the same effect as with the low network throughput scenario, making consensus unachievable and hindering transaction throughput. In contrast, any of the network nodes may be exposed to such an attack, not only nodes suffering from low network throughput, all though they would be more susceptible.

%This could be a severe vulnerability regarding the network, if there is little overlap between nodes' quorum slices, making such an attack practical. In regards to RPCA, the UNL overlap requirement of 90\% should make such an attack infeasible. The attack however could be very relevant in terms of SCP, if users are selective in which nodes they want to trust. It is not clear whether such a system could effectively defend itself towards the attack, without any special incentive or centralized intervention.  


%\subsection{Hybrid}



%In an effort to consolidate the benefits of both Nakamoto and BFT style consensus, recent years has seen the development of hybrid style consensus algorithms, like BFT-based POW and BFT-based POS. Concrete examples of these types of algorithms are Byzcoin consensus and Tendermint, respectively. These algorithms typically provide consensus in linear communication complexity\footnote{In terms of the total amount of nodes in the network, $n$. In terms of the size of the consensus group created, m, the complexity is $\Theta(m^2)$. This is similar to most BFT style consensus algorithms.}, using a three step BFT style process to reach consensus, while using mechanisms from Nakamoto style consensus algorithms for leader election. This scheme allows for immediate finality, while also providing Sybil attack resistance, enabling the consensus algorithms to work in a permissionless setting. The consensus algorithms are proposed to be able to scale better than standard Nakamoto consensus algorithms, but at the cost of reduced Byzantine fault tolerance, requiring a supermajority of honest nodes for safety. 

%\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}

%The hybrid consensus algorithm identified make similar synchronization assumptions to that of BFT style consensus algorithms. In particular, Byzcoin assume weak synchrony, while Tendermint assume partial synchrony. Both equate to messages at some point being bound by some upper message delay $\Delta$, to enable liveness. In times of asynchrony, while preserving safety, the consensus algorithms' transaction throughput may suffer significantly. For the relevant setting, with potential high communication delay and periods of asynchrony, this may be problematic.

%\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput? }

%A potential pain point of making the transition from Nakamoto style consensus to a hybrid approach, is the increased susceptibility to DDOS attacks. Similar to BFT style consensus algorithms, the hybrid approach is leader-centered, and need to maintain a stable leader to provide high performance. Combined with limited network throughput, this may further hinder transaction throughput.


% Centralization concerns?

%\subsection{Crash Tolerant}

%The only crash tolerant consensus algorithm identified, Raft, provide consensus in a single communication step, with the optimal communication complexity of $\Theta(n)$. It also provides deterministic finality. The main caveat related to crash tolerant consensus algorithms is that they cannot tolerate Byzantine faults; there is inherent trust that the current leader follows the protocol. If not, safety cannot be guaranteed. Disregarding Byzantine faults, Raft tolerate up to 50 \% crashed nodes. Overall, this limits Raft's use to that of private blockchain systems, where there is high degrees of trust among stakeholders. 

%\subsubsection{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}

%Raft furthermore relies on synchronization assumptions regarding the underlying network, similar to that of BFT style consensus algorithms. In particular, it assumes a known broadcasting latency, which is then used to determine an election timeout interval. This may be problematic in terms of a network with high communication latency and poor network throughput; a too low latency parameter and the network cannot make progress, too high and transaction throughput is throttled. 

%Another consideration is that Raft's communication pattern is completely leader-centered; during normal operation, the leader continuously broadcasts messages to the rest of the network, while follower nodes only respond to the messages they receive. It is therefore highly important that the leader node has sufficient network throughput and computational resources, in order for the leader not to become a bottleneck in terms of performance. In regards to nodes with low network throughput, systems designers would need to consider ways to mitigate this. A potential solution could be to disallow such nodes from leader election, at the cost of the system's robustness.

%\subsubsection{RQ2: What consensus models are able to provide security in an environment with limited network throughput? }

%In terms of security, Raft suffers from the same DDOS susceptibility as BFT style consensus algorithms. The consensus algorithm need to maintain a stable leader to provide liveness, and such, continuous DDOS attacks targeting leaders can hamper transaction throughput. This may be further exasperated by nodes having limited network throughput, if not adequately mitigated.  


==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/implementation.tex <==
%\section{Research Implementation}
%\label{sec:method}


%This section presents the paper's research methodology. Specifically, 

%The study's research questions are defined, as well as its literature search, paper screening and classification scheme. 

%\subsection{Definition of Research Questions}

%To specify the scope of the study, the following research questions were defined: 

%\todo{Research questions mentioned trice, remove?}
%\textbf{RQ1:} What consensus models are able to provide integrity in an environment with limited network throughput?

%\textbf{RQ2:} What consensus models are able to provide security in an environment with limited network throughput?


% OG Research questions

%\textbf{RQ1:} What mechanisms enable consensus algorithms to provide high transaction throughput in SCM blockchain systems?

%\textbf{RQ2: }What mechanisms enable consensus algorithms to ensure security in SCM blockchain systems? \begin{itemize}
    %\item[-] \textit{RQ2-1:} What mechanisms enable consensus algorithms to ensure correctness in SCM blockchain systems?
    %\item[-] \textit{RQ2-2:} What mechanisms enable consensus algorithms to ensure liveness in SCM blockchain systems?
%\end{itemize}

%\textbf{RQ3:} What mechanisms enable consensus algorithms to provide a high degree of decentralization in SCM blockchain systems?



% Research questions:

% Network model needed

% Consortium -> Not decentralized

% Minimum network speed to deliver on high reliability. Look at IBM taxonomy. Test with network parameters. 

% Rq1: What are the minimum throughput / performance for the consensus model to provide sufficient integrity?

% Rq2: What are the minimum throughput / performance in which the consensus model can defend against *certain* security attacks?

% Grey literature -> Arxiv. Same search query. 


%\subsection{Conducting the search}

%In order to gather research papers related to consensus algorithms, search queries are defined and executed at a set of scientific databases. 
\subsection{Data collection}
We followed the systematic mapping study guideline proposed by \citep{RN14}. The search query \textit{"Blockchain AND Consensus Algorithm"} was used to identify papers related to consensus in blockchain systems. The query was executed at Oria \citep{Oria}, a search engine aggregating research papers from scientific databases, including IEEE Xplore, Springer, ACM Digital library, and Scopus. We included only peer-reviewed research papers in this round of search. Furthermore, to also gain insight into the current non-peer-reviewed literature, the aforementioned search query was also executed towards Arxiv.org. This combined search is meant to provide a holistic view of the current literature on consensus mechanisms applicable to blockchain systems.
To exclude irrelevant papers, we first read through the papers' titles and abstracts. Papers that did not explicitly mention consensus algorithms were excluded. Papers that were not available online were also excluded. Furthermore, we excluded any paper that does not provide an adequate description of the algorithm or sufficient security analysis. 

A total of 2151 papers were identified via the Oria search engine. Through disregarding non-peer-reviewed papers, the total was narrowed down to 451 papers. We then read through the papers' titles and abstracts to exclude any paper that did not explicitly mention consensus algorithms and got 81 papers. Of these 81 papers, 63 papers were identified as studies that presented consensus algorithms.  Regarding the search executed at  Arxiv.org,  a  total of  103  papers were identified.  The papers were analyzed in the same manner as with the  Oria search. To get representative consensus algorithms, We only include consensus algorithms if they were discussed in more than one paper. We end up with a total of 25 consensus algorithms to analyze.


%Collectively, the remaining papers were then analyzed, excluding any papers related to consensus algorithms already identified by related work. Furthermore, papers claiming to provide novel consensus models\footnote{Novel meaning not discussed in the related work. See section \ref{sec:related_work}.}, but which did not provide adequate description or security analysis, were also excluded. Following this criteria, a total of 5 novel consensus algorithms were identified, summarized below.

%\subsection{Screening for relevant papers}

%Inclusion and exclusion criteria allow for excluding papers which are not relevant to answering the study's research questions \citep{RN14}.
 
%Following this initial gathering, papers were identified as either related work, or papers potentially presenting novel consensus mechanisms. The identified related work constitutes this paper's related work section. The remaining papers were then analyzed, excluding any papers not claiming to contribute a novel consensus model. 

\subsection{Data analysis}

%Central to discussing the integrity and security of consensus mechanisms are the properties of \textit{safety} and \textit{liveness}, established by \citet{RN48}. \textit{Safety} means that incorrect operations cannot happen during execution. \textit{Liveness} mean that correct operations will eventually be executed by the system. Safety is comparable to the correctness of the consensus algorithm. In particular, according to the assumptions made by the consensus model, there is no sequence of events in which the system can enter an erroneous state. As an illustrating example, despite the presence of a adversarial environment, the Nakamoto consensus scheme is able to ensure eventual consistency within the Bitcoin network, given that the assumption of an honest majority within the network holds. Conversely, liveness is comparable to the consensus algorithm's ability to make forward progress. While it is essential that the algorithm is correct, if the algorithm cannot provide liveness, it cannot be effectively utilized in a practical setting. As another illustrating example, despite interference from adversarial parties, honest actors participating in the Nakamoto consensus are eventually able to agree upon a set of transactions, given an honest majority within the network. 

Our classification is based on qualitative analysis and uses a classification scheme differing from \cite{RN14} because none of the identified papers sufficiently covered the topic of consensus in low throughput networks. To classify performance of the consensus algorithms and to answer RQ1, we applied the metrics shown in \autoref{tab:classification_scheme}. 

\begin{itemize}

\item Reference \citep{RN52} define read and transaction latency and read and transaction throughput as essential performance metrics. In this study, we are specifically interested in evaluating consensus mechanisms in relation to a blockchain system affected by low network throughput, distributed over a greater geographical area. Thus, the particular focus of the classification is attributed to communication-related costs, in the form of \textit{consensus latency} and \textit{communication complexity}.

\item To avoid the impossibility result \citep{RN40}, one can assume that the underlying communication network is synchronous. However, the network may be particular asynchronous \citep{RN46} because of the limited network throughput. Thus, the consensus algorithms' \textit{timing assumptions} are also included as a metric. The timing assumptions made by consensus algorithms can be categorized accordingly. 
\begin{itemize}
    \item \textbf{Synchronous:} There exist a known fixed upper bound $\Delta$ on the message delay between peers within the network. 
    \item \textbf{Partial Synchronous:} Either of the following statements holds: 
    
      \begin{enumerate}[i]
      \item There exists an upper bound $\Delta$ on the message delay between peers within the network, but it cannot be known a priori.
      \item There exists an upper bound $\Delta$ on the message delay between peers within the network, but it does not hold before an unknown point of time $T$.
      \end{enumerate}
   \item \textbf{Asynchronous}: There is no known fixed upper bound $\Delta$ on the message delay between peers within the network.
\end{itemize}

\item \textit{Byzantine fault tolerance} and transaction \textit{finality} are included, highlighting the algorithms' resilience towards adversarial attacks, as well as transaction confirmation time. A consensus algorithm's transaction finality is the algorithm's guarantee that committed transactions cannot be reversed. Some consensus algorithms providing probabilistic finality, e.g., Nakamoto style consensus, favor availability over strong consistency. Other consensus algorithms providing immediate finality, e.g., BFT style consensus, need strong consistency to enforce this, thus sacrificing the system's availability during network partitioning.  

\end{itemize}


% New table formatting to fit page
\begin{table}[h]
    \centering
     \begin{tabular}{lp{5cm}}
        Metrics & Description \\\hline
        Consensus latency &  Number of Round-trip time (RTT) needed to complete a round of consensus.  \\
        Communication complexity &  Number of messages needed to complete a round of consensus.  \\
        Timing assumptions &  Timing assumptions made by the consensus model related to the underlying network. This relates to a synchronous, partial synchronous or asynchronous network.  \\
        Byzantine Fault Tolerance & The percentage of adversarial control in the network, in which the consensus model can resist double spend attacks.  \\
        Finality & The assurance that transactions committed will not be reverted. Either immediate or probabilistic.  \\
        
    \end{tabular}
    \caption{Metrics to measure performance and to answer RQ1}
    \label{tab:classification_scheme}
  
\end{table}

%\begin{table}[h]
%    \centering
%     \begin{tabular}{lp{10cm}}
%        Category & Description \\\hline
%        Consensus latency &  Number of Round-trip time (RTT) needed to complete a round of consensus.  \\
%        Communication complexity &  Number of messages needed to complete a round of consensus.  \\
%        Timing assumptions &  Timing assumptions made by the consensus model related to the underlying network. This relates to a synchronous, partial synchronous or asynchronous network.  \\
%        Byzantine Fault Tolerance & The percentage of adversarial control in the network, in which the consensus model can guarantee safety.  \\
%        Finality & The assurance that transactions committed will not be reverted. Either immediate or probabilistic.  \\
        
%    \end{tabular}
%    \caption{Classification scheme}
%    \label{tab:classification_scheme}
  
%\end{table}



%\subsection{Data extraction}

%Based on the classification scheme stated, the identified consensus models were categorized. The results of this process is described in \autoref{sec:study_results}. 

%\subsection{Security considerations in blockchain systems}

%\label{subsec:security}


%When designing a blockchain system, there are several security aspects to considers. 
To answer RQ2, we first identified core security issues related to the blockchain system based on \cite{RN17} and \cite{RN30}. The identified security issues are shown in \autoref{tab:background_security_considerations}. In terms of the SCM setting, with a permissioned blockchain system affected by limited network throughput, not all security issues listed in \autoref{tab:background_security_considerations} are relevant. For example, given that participants in the system are authenticated, a Sybil attack can effectively be combated. In an authenticated setting, aspects like user anonymity and transaction unlinkability are deemed irrelevant. We excluded irrelevant security issues and classified the consensus algorithms based only on double-spend attacks, balance attacks, Long-range attacks, p + Epsilon attacks, DDOS attacks, and BGP attacks.

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{4cm}p{13cm}}
         Name & Description \\\hline
         Consistency & Which approach will the system utilize to ensure the consistency of the system's ledger?  \\
         Tamper-Resistance & Is the system able to ensure the integrity of the ledger? \\
         Byzantine Fault Tolerance & To which an extent do the system need to tolerate Byzantine faults, e.g. adversarial nodes?  \\
         Sybil attack & How will the system protect against malicious actors creating multiple fake identities, attempting to outvote an honest majority?  \\
         Double spend attack & How will the system prevent nodes spending the same currency for two separate transactions? Specifically related to cryptocurrency systems.  \\
         Long-Range attack & To which extent is the system vulnerable to Long-Range attacks; forking the blockchain at its genesis block and privately building an alternative chain?  \\
         P+ Epsilon attack & To which extent is the system vulnerable to P+ Epsilon attacks; taking advantage of the dominant strategy among network participants, leveraging non-altruistic participants against the system? \\
         Balance attack & To which an extent is the system vulnerable to balancing attacks; splitting the network into sub-networks, delaying transactions and performing double spend attacks? \\
         Border Gateways Protocol (BGP) Hijacking & How will the system handle adversarial attacks against the network's routing mechanisms; partitioning the network or delaying block propagation? \\
         Distributed-Denial-of-Service (DDOS) susceptibility &  To which an extent is the system susceptible to DDOS attacks, in terms of impact upon safety and liveness? Especially relevant for leader based consensus models. \\ 
         Degree of centralization & To which an extent is the system centralized around a subset of participants? This may have implications on various double spend attacks, as well as DDOS susceptibility.   \\
         User anonymity & Are participants of the system able to partake in transactions while staying anonymous?\\
         Transaction confidentiality & To which extent are transactions kept confidential? \\
         Transaction unlinkability & To which extent is it possible to link a group of transactions to a specific identity?\\
    \end{tabular}
    \caption{Security considerations for blockchain systems}
    \label{tab:background_security_considerations}
\end{table*}

%The concept of \textit{consistency} in relation to a blockchain system refers to its ability to keep the ledger consistent across the participants of the network \citep{RN17}. As stated by the CAP theorem \citep{CAP}, a distributed system cannot guarantee strong consistency, availability and partition tolerance simultaneously. Blockchain systems may therefore utilize different approaches in terms of consistency. In particular, common approaches implemented by  blockchain system are strong consistency, ensuring that nodes keep the same ledger at all times, and eventual consistency, in which nodes may have differing ledgers at some specific point of time, but eventually become consistent. Here, strong consistency comes with the trade-off of reduced availability in the event of network partitioning, while eventual consistency introduce the need for conflict resolution, should there be a dispute regarding which ledger is correct. 

%\textit{Tamper-Resistance}, in terms of a blockchain system, refers to the system's ability to ensure the integrity of the information stored in its ledger, during and after block generation \citep{RN17}. Specifically, when new blocks are propagated within the system, the system's nodes need to be able to assert the validity of the transactions contained within the block. Adversaries may in particular attempt to modify a transaction to be included in the new block, or transactions already part of the ledger. Both are conventionally avoided by the use of strong cryptographic mechanisms, utilizing secure hash functions to assess that the integrity of transactions and blocks are not compromised, as well as digital signatures, ensuring that the transaction's origin are who they claim to be. 

%Essential to system is its requirements towards \textit{Byzantine Fault Tolerance}. In a trustless peer-to-peer network, some degree of Byzantine fault tolerance is needed, to protect against arbitrary or malicious behavior by network participants.  The degree may then again vary depending on the setting of the system, whether it is permissioned or permissionless. Commonly labeled as the \textit{51\% attack}, malicious actors have been conjectured to have the ability to override honest transactions in cryptocurrencies like Bitcoin or Ethereum, given a majority of the hashing power of the network. This is further applicable to traditional BFT consensus models, where the system commonly assumes a maximum number of faulty nodes $f$, providing implications on the total number nodes required for consensus, and thus the scalability of the model.  

%Another common attack vector within P2P systems is the \textit{Sybil attack}, where malicious actors create multiple fake identities, attempting to increase their influence upon the network. This is elegantly addressed in Nakamoto's Proof-of-Work scheme \cite{Nakamoto_Bitcoin_POW}, linking voting power to hashing power, thus making Sybil attacks ineffective. It is also addressed in permissioned blockchain systems, requiring all participants of the network to be authenticated, linking each identity to real world entities. The attack is consequently especially relevant in permissionless settings. 

%Related to cryptocurrencies like Bitcoin, there is the \textit{Double spend attack}. This specifically refers to the action of spending a single amount of currency twice, i.e. in two separate transactions. In Bitcoin, this is partially dealt with by ensuring the integrity of transactions and including digital signatures, ensuring that parties partaking in the transaction are who they claim to be. Furthermore, transactions are only assumed to be confirmed after $k$ succeeding blocks, making the chance of reversing a previously committed transaction small. However, since the system's consensus termination is probabilistic, the potential for a fork is still there, enabling a double spend attack. This is further highlighted through the \textit{Blockchain Anomaly} \citep{RN38}, showing the impossibility of guaranteeing that certain committed transactions will not be removed from the main chain in the future. 

% start at early point of blockchain. build blocks privately, can forge time stamps to allow quicker generation of blocks. Publish larger chain later, causing double spends.
%Some blockchain systems may also be vulnerable to a \textit{Long-Range attack} \citep{RN55}. Related to other majority consensus attacks, instead of attempting to hijack $k$ block confirmation limit, the attacker forks the chain at a much earlier point. The alternative chain is then privately mined upon by the attacker. \citet{RN55} proposes that in some types of blockchain systems, e.g. earlier versions of the Ethereum client, the attacker can take advantage of the fact that they are the only entity contributing to the alternative chain, accelerating the rate in which blocks are generated. This can then be used to overtake the main chain, enabling double spend attacks. \citet{RN55} goes on to explain that blockchain systems may protect against such attacks by limiting the variability among alternative chains. 

%Another possible attack, the \textit{P+ Epsilon attack}  \citep{RN54}, leverages non-altruistic participants in the attacker's favor. By promising to provide some kind of reward, denoted $\epsilon$, the attacker can align other participants' incentives according to their own, creating a dominant strategy within the network. This then allows the attacker to carry out their goals, despite not controlling a majority of the network themselves, assuming that altruists do not constitute a majority within the network. The attacker may later on not pay out the reward promised, reaping the profit of the attack all by themselves \citep{RN30}.  

%The \textit{balance attack} constitutes another flavor of the double spend attack, allowing malicious actors to force double spend attacks despite an honest majority, given sufficient network delay. \citet{RN39} provide a theoretical analysis of the attack and demonstrate its feasibility through experimental results, utilizing the Corda blockchain platform. The attack provides a valid security concern regarding use of proof-of-work based consensus schemes in blockchain systems with considerable network delay. 

%\textit{Border Gateways Protocol Hijacking} (BGP) involve an attacker taking control over parts of the Internet routing infrastructure utilized by the blockchain system \citep{RN53}. By controlling key parts of the routing mechanisms of the network, attacker may be able to both partition the network, isolating participants from communicating with their peers, as well as significantly delaying block propagation. \citet{RN53} goes on to demonstrate the feasibility of both types of attacks. Similar to that of a balance attack, this can be used to perform double spends in certain types of blockchain systems. 

%Blockchain systems may also be susceptible towards \textit{distributed denial of service} (DDOS) attacks. In particular, if the consensus model is leader-based, the system's liveness may be threatened. By overloading the leader with incoming traffic, this may prevent them from carrying out the consensus algorithm and thus impact the transaction throughput of the system. Furthermore, DDOS attacks may have implications on the number of faulty nodes of the system. This may impact the consensus scheme directly, in the case of BFT algorithms. It may also impact it indirectly, by altering the distribution of available computational resources, shifting the balance of power in the case of Proof-of-Work based consensus algorithms. 

%To conclude, the \textit{degree of centralization} of a blockchain system may impact its security. Within certain consensus models, centralizing power within a subset of the nodes have inherent risks. It may provide incentive for DDOS attacks, as powerful nodes have greater influence upon the network, thus increasing the impact of an attack. It may furthermore heighten the risk of collusion, reducing the number of nodes for an adversary to corrupt. This may then lead to potential abuse of power, in form of double spend attacks.

%Additionally, \citet{RN17} propose the security properties of \textit{user anonymity}, \textit{transaction confidentiality} and\textit{transaction unlinkability}. These properties all relate to the privacy of participants partaking in the blockchain system, protecting their identity and the confidentiality of the data they commit to the blockchain. This may be of great benefit in the setting of financial system, e.g. a cryptocurrency like Bitcoin, in which lack of privacy may enable attacks against lucrative targets. In an authenticated setting, it may be less applicable. 



==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/introduction.tex <==
\section{Introduction}
% Motivate for blockchain as a technology and its benefits
Blockchain has evolved significantly since its initial roots from Bitcoin and has seen adoption with novel use of the technology for healthcare \cite{mettler2016blockchain}, banking \cite{peters2016understanding}, control systems \cite{stanciu2017blockchain}, and SCM \cite{chang2020blockchain}. In SCM systems, different actors are working together to deliver timely and quality products to their customers. A consensus algorithm used in SCM systems shall provide high transaction throughput to take advantage of vast amounts of IOT sensor data. Furthermore, it would need to function well in an environment with varying network delays. Some nodes, e.g., nodes to collect and transfer temperature data of fresh food on trucks or vessels, may have poor or no internet connection. The blockchain system will be subject to the CAP theorem \citep{CAP}, which is challenging, given high requirements towards transaction throughput and the constraint caused by an unstable network environment. 

This study aims to study to which degree existing consensus algorithms can provide integrity and security with limited network throughput and low network quality. Our primary research hypothesis theorizes that there is little empirical knowledge of blockchain applications' effectiveness with limited network throughput concerning the consensus mechanisms. We performed a mapping study and covered published and preprint articles. Our study aimed at answering the following research questions.

\textbf{RQ1:} How well existing consensus algorithms can provide integrity in an environment with limited network throughput?

\textbf{RQ2:} How well existing consensus algorithms can provide security in an environment with limited network throughput?


We identified and analyzed 25 consensus algorithms qualitatively in this study. The results show that many existing consensus algorithms are unfit for use in an environment affected by varying network throughput. Some consensus algorithms which assume a partially synchronous network can provide integrity in events of asynchrony. However, their transaction throughput may be significantly reduced when faced with targeted denial-of-service attacks. Consensus algorithms that do not make synchronization assumptions, adapted to an asynchronous network, may avoid both.  

The remainder of the paper is organized as follows. 
Section 2 lists related work. 
Section 3 explains the research design and implementation. 
Section 4 present the research result.
Section 5 discusses the results and Section 6 concludes the study.


==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/relatedWork.tex <==
\section{Related Work}
\label{sec:related_work}

%This section of the paper aims to identify existing literature related to consensus algorithms used within blockchain systems. The papers described are the outcome of a systematic search, described in \autoref{sec:method}. In particular, 18 related studies were identified. The studies were then assessed, omitting any studies which were not found to be within the scope of the paper. After revision, a total of 13 studies were included, described in \autoref{tab:relevant_studies}.




%\begin{table}[h]
 %   \centering
 %    \begin{tabular}{llll}
 %       ID & Reference & ID & Reference \\
 %       1 & \citeauthor{RN21} \citeyear{RN21} & 8 & \citeauthor{RN24} \citeyear{RN24}\\
 %       2 & \citeauthor{RN18} \citeyear{RN18} & 9 & \citeauthor{RN16} \citeyear{RN16} \\
  %      3 & \citeauthor{RN19} \citeyear{RN19} & 10 & \citeauthor{RN23} \citeyear{RN23} \\
  %      4 & \citeauthor{RN22} \citeyear{RN22} & 11 & \citeauthor{RN26} \citeyear{RN26} \\
  %      5 & \citeauthor{RN25} \citeyear{RN25} & 12 & \citeauthor{RN27} \citeyear{RN27}  \\
  %      6 & \citeauthor{RN17} \citeyear{RN17} & 13 & \citeauthor{RN31} \citeyear{RN31} \\
  %      7 & \citeauthor{RN30} \citeyear{RN30} & &  \\
 %   \end{tabular}
 %   \caption{Relevant related studies}
  %  \label{tab:relevant_studies}
  
%\end{table}

%Following the rise of Bitcoin, the underlying blockchain technology received great interest. A core concept of the blockchain is the consensus algorithm, providing a secure way for participants in the network to agree upon transactions, without the need for a central authority. Following Bitcoin's Nakamoto consensus model \citep{Nakamoto_Bitcoin_POW}, other consensus algorithms have been proposed. 

Studies, e.g., \citep{RN21, RN18, RN19, RN22, RN25}, have focused on reviewing the state of the art consensus algorithms.
\citep{RN21} defined a five-component framework for categorizing blockchain consensus algorithms, provided a comprehensive review of current consensus algorithms, and evaluated the algorithms' performance according to their fault tolerance and throughput. \citep{RN18} analyzed the algorithm's throughput, mining incentive, decentralization, and security challenges. \citep{RN25} provided a game-theoretic point of view and looked at the mining incentive provided by different consensus algorithms. \citet{RN19} evaluated the Proof-of-Work (PoW) scheme of cryptocurrencies like Bitcoin and Ethereum according to traditional Byzantine consensus algorithms, and provided insight into PoW specific security challenges, like the Bitcoin anomaly and balancing attacks. \citep{RN22} provided an extensive mapping of consensus algorithms, according to their architecture and paradigm, and highlighted fundamental differences between public and private blockchain systems, and showed how this impacts the algorithms' applicability in these specific types of systems. 

Other studies, e.g., \citep{RN17, RN30}, have focused on security challenges related to using using blockchain technology. In particular, the studies highlighted the security implications the choice of consensus algorithm has upon the overall blockchain system. \citep{RN17} provided a comprehensive overview of security and privacy aspects of blockchain technology, defined core security properties, and described existing security techniques. \citet{RN30} assessed major Nakamoto style consensus algorithms against the 51\% attack, as well as other major security threats towards blockchain systems, and reviewed current mitigation techniques. 

Both industry and academia have shown great interest in assessing new use cases for blockchain technology, following its success within the cryptocurrency space \citep{RN24, RN16, RN23, RN26}. \citet{RN24} provided a \textit{vademecum} to guide designers in their decisions for when and how to apply blockchain technology to their specific use case. Reference \citep{RN16} presented a systematic review of blockchain within the energy sector and discussed its limitations and potential use cases. Reference \citep{RN23} reviewed current blockchain initiatives and highlighted domains having real-world technology adoption. \citet{RN26} presented a comprehensive analysis of the state of the art consensus algorithms and their appropriateness related to cyber-physical systems. In particular, the authors outlined domain-specific challenges for supply chain management blockchain systems.

Another exciting research area has been the interconnection of blockchain technology and IOT systems. Several studies, e.g., \citep{RN27, RN31}, have been dedicated to describing the state of the art IOT blockchain systems and their challenges. Reference \citep{RN27} provided an extensive analysis of key components of IOT blockchain systems and promising consensus schemes and reviewed major IOT blockchain projects. \citep{RN31} reviewed core security issues related to IOT systems and how blockchain technology might be applied to solve some of these issues. The research goals of the related studies mentioned above are summarized in \autoref{tab:relevant_studies_characteristics}.  Furthermore, the consensus algorithms they discussed are summarized in \autoref{tab:relevant_studies_consensus_algos}.
\renewcommand{\arraystretch}{1.25}

\begin{table*}[t]
    \centering
     \begin{tabular}{p{6cm}ccccccccccccc}
        Reference ID & \cite{RN21} & \citep{RN18} & \cite{RN19} & \cite{RN22} & \cite{RN25} & \cite{RN17} & \cite{RN30} & \cite{RN24} & \cite{RN16} & \cite{RN23} & \cite{RN26} & \cite{RN27} & \cite{RN31} \\\hline
        %\multicolumn{14}{l}{\textbf{Research goals}} \\\hline
        Review existing consensus algorithms & x & x & x & x & x & x & x & x & x & x & x & x & x \\
        Review and analyze current blockchain projects &  &  & x &  &  &  &  & x & x & x &  & x & x \\
        Security analysis &  & x & x &  & & x & x &  &  &  &  &  &  \\
        Provide analysis framework & x & x &  &  &  &  &  &  &  &  &  &  &  \\
        Present domain specific use cases &  & &  &  &  &  &  & x & x & x & x & x & x \\
        %\multicolumn{14}{l}{\textbf{Number of papers included}} \\\hline
        %Potentially Relevant Papers &  &  &  &  &  &  &  &  &  &  & 454 & 12 & 13 \\
        %Relevant Papers Included &  &  &  &  &  &  &  &  &  &  & 122 & 12 & 13 \\
        %\multicolumn{14}{l}{\textbf{Consensus Algorithms}} \\\hline
        %Number of consensus algorithms included & 22 & 12 & 4 & 66 & 22 & 12 & 3 & 12 & 10 & 10 & 25 &  &  \\
    \end{tabular}
     \caption{Research goals of related studies }
     \label{tab:relevant_studies_characteristics}
\end{table*}
%Edit: Reduce table text to fit

\begin{table*}[t]
    \centering
    \begin{tabular}{p{6cm}ccccccccccccc}
        Reference ID & \cite{RN21} & \citep{RN18} & \cite{RN19} & \cite{RN22} & \cite{RN25} & \cite{RN17} & \cite{RN30} & \cite{RN24} & \cite{RN16} & \cite{RN23} & \cite{RN26} & \cite{RN27} & \cite{RN31} \\\hline
    
     Proof of Work (PoW) & x & x & x & x & x & x & x & x & x & x & x & x & x \\
     Proof of Stake (PoS) & x & x &  & x & x & x & x & x & x & x & x & x & x \\
     Delegated Proof of Stake (DPOS) & x & x &  & x &  & x & x & x & x & x & x &  & x \\
     Proof of Authority (PoAuth) & x &  &  & x &  & x &  & x & x & x &  & x &  \\
     Proof of Elapsed Time (PoET) & x & x &  & x & x & x &  & x & x &  & x &  &  \\
     Proof of TEE-Stake (PoTS) & x &  &  &  &  &  &  &  &  &  & x &  &  \\
     Proof of Retrievability (PoR) & x &  &  & x & x &  &  &  &  &  &  &  &  \\
     Proof of Weight (PoWeight) &  & x &  &  &  &  &  &  &  &  &  &  &  \\
     Proof of Burn (PoB) &  & x &  & x & x &  &  &  & x & x & x & x & x \\
     Proof of Capacity (PoC) &  & x &  & x &  &  &  &  & x & x & x & x & x \\
     Proof of Importance (PoI) &  & x &  & x &  &  &  & x &  & x & x & x &  \\
     Proof of Authority (PoA) &  & x &  & x & x &  &  &  & x & x &  &  &  \\
     Practical Byzantine Fault Tolerance (PBFT) & x & x & x & x &  & x &  & x & x & x & x & x & x \\
     Delegated Byzantine Fault Tolerance (Delegated BFT) &  & x &  & x &  &  &  &  &  &  & x &  &  \\
     Democratic Byzantine Fault Tolerance (Democratic BFT) &  &  & x &  &  &  &  &  &  &  &  &  &  \\
     Byzantine Fault Tolerant State Machine Replication (BFT-SMART) &  &  &  & x &  &  &  &  &  &  &  &  &  \\
     Honey-Badger Byzantine Fault Tolerance (Honey-Badger BFT) & x &  &  & x &  & x &  &  &  &  &  &  &  \\
     Ripple Protocol Consensus Algorithm (RPCA) & x &  & x & x &  &  &  & x &  & x & x & x &  \\
     Stellar Consensus Protocol (SCP) &  &  &  & x &  &  &  & x &  &  &  &  &  \\
     Byzantine Fault Tolerance based Proof of Work (BFT-based POW) &  &  &  &  & x &  &  & x &  &  &  & &  \\
     Byzantine Fault Folerance based Proof of Stake (BFT-based POS) & x &  &  & x & x & x &  & x &  &  &  &  & \\
     Paxos &  &  &  &  &  &  &  &  &  &  & x &  &  \\
     Raft &  &  &  & x &  & x &  & x &  &  & x &  &  \\
    \end{tabular}
    \caption{Consensus algorithms  in related studies}
     \label{tab:relevant_studies_consensus_algos}
\end{table*}


%%%%%%%% Observations and conclusions %%%%%%%%%%%%%%


%Throughout the related studies, larger focus has been dedicated to presenting state of the art consensus algorithms, current project initiatives and the potential use cases blockchain technology has in certain domains. Consensus algorithms presented mainly fall into the groups of Nakamoto style consensus algorithms, including Proof of Work and Proof of Stake variants, as well as Byzantine Fault Tolerant algorithms, including Practical Byzantine Fault Tolerance and the Ripple Protocol Consensus Algorithm. 

%Especially relevant to this paper, \citet{RN26} highlight the use case of applying blockchain technology in the context of supply chain management systems; providing the benefits of traceability, accountability and improved information sharing  to the transfer of goods between stakeholders. The authors goes on to summarize several of the algorithms which have been proposed for usage within the domain, including Proof of Work, several variants of Proof of Stake, as well as Practical Byzantine Fault Tolerance and Ripple Protocol Consensus Algorithm. This matches the general trend previously described.     
None of the related studies highlight the challenge of consensus in environments with varying network delays. In particular, in the context of supply chain management systems, real-world scenarios often involve entities transporting goods over larger geographical areas, with periods of poor or no internet connection. To deliver on the promises of traceability, accountability, and improved information sharing, SCM blockchain systems' underlying consensus algorithm must allow for efficient data sharing between stakeholders, despite participants being affected by varying network delays. Therefore, assessing the state of the art consensus algorithms' performance under such an environment is essential to find suitable consensus algorithms for SCM blockchain systems. Furthermore, such an analysis may uncover the need for designing novel consensus mechanisms if current mechanisms are found insufficient for the use case.

% None of them focus on network with variying / high network delay. For SCM systems, real world scenario oftentimes involve entities traveling over larger geographical areas, with periods of poor or no internet connection. In order to efficiently supply data to stakeholders in a secure manner, one must pick a consensus algorithm appropriate for such an environment. 

% Assessing what type of consensus algorithm is needed, to maximize transaction throughput, while keeping sufficient level of security and decentralization.


% What constitutes a good consensus algorithm for an environment with an unstable network?

% Number of RTT for each round of consensus?
% Amount of data needed to receive per round of consensus (i.e. data overhead imposed by the algorithm)?
% Estimated throughput, given sufficient network?

% Tradeoff between numbers of messages sent and number of communication steps. More steps, lead to more RTT, increase time to find solution, decrease throughput. More messages per step can decrease number of step needed to take. Also impose extra processing costs. 

% Given low bandwith, want to minimize amount of data sent/received. 

% Amount of data needed to be sent = Size of message * ( (Number of steps) * Message sent per step)

% Participants are far between -> High latency, meaning RTT is high and each communication step is expensive. Throughput is therefore most benefited from an algorithm which has few communication steps. 

% Ex: PBFT -> 3 full communications steps per round.

% Ex: Raft -> Leader sends out message continuously (including NIL messages) at fixed time interval. Can over stimulate a limited network capacity, possibly okay 

% Ex: POET (proof of work based) -> Single (?) step, plus propagation. Need however to do the work, e.g. solve puzzle, which imposes its own time cost. 



% 




% Idea: Do not use the edge node as validator, rather just as a transaction producer. Do not need to participate in consensus part (?). Perhaps a pre-condition. 












==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/researchDesign.tex <==
\section{Research Design and Implementation}

%This section presents the paper's research design. In particular, it states the purpose of the research project, its contributions, the research methods applied, as well as the participants involved. Finally, the deliverables of the project are also assessed. 

%\subsection{Purpose}

% Blockchain is an emerging technology, which have many usecases, including supply chain management

% There are multiple frameworks for creating blockchain solutions at a enterprise level. However, they are not deemed mature enough 

%Blockchain is an emerging technology, tracing back to the rise of Bitcoin and other cryptocurrencies. Recent efforts have focused on other use cases of the technology, including applications within international banking, healthcare, as well as supply chain management (SCM). In particular, SCM has been deemed a promising area for applying blockchain technology, as it can enable the transparency and traceability of goods in a decentralized manner. In combination with IOT sensor data, stakeholders can fully document a goods' journey across different actors, ensuring ethical operation and accountability. 

%There currently exists multiple frameworks enabling the creation of enterprise level blockchain solutions, including platforms like Hyperledger, Corda and Quorum. However, a large degree of these frameworks are targeted at financial services. While some of these platforms provide tools for developing blockchain-based solutions for SCM, they have low maturity and are not capable of supporting core business goals; The tracing and delivery of goods over large geographical areas, involving numerous stakeholders and governance sectors. Furthermore, the solutions are not adept at handling vast amount of IOT sensor data, served over a potentially unstable network, something which poses new challenges. 

%At the core of blockchain technology is the consensus algorithm, enabling participants to reach agreement in a decentralized fashion. Related to this, numerous novel consensus algorithms have been proposed in recent years, attempting to improve upon the original Proof-of-Work scheme proposed by Nakamoto \citep{Nakamoto_Bitcoin_POW}. In particular, given the rise of permissioned, enterprise blockchain applications, new consensus algorithms can take advantage of these systems' differing security requirements, improving scalability and transaction throughput. 

%Providing a suitable platform for SCM blockchain systems is a multifaceted problem. Part of the solution will be the selection of core consensus mechanisms. A consensus algorithm used in such systems would need to provide high transaction throughput, in order to take advantage of vast amounts of IOT sensor data. Furthermore, it would need to function well in a network with varying network throughput, as nodes may have poor or no internet connection. The blockchain system will subject to the CAP theorem \citep{CAP}, and such a balance between consistency, availability and partition tolerance must be reached. In particular, this may be deemed challenging, given an unstable network environment and high requirements towards transaction throughput. 

This study aims to provide insight into core mechanisms of the state of the art consensus algorithms and how they relate to SCM blockchain systems in an enterprise setting with multiple stakeholders affected by varying network throughput. 

%The system can be seen as an asynchronous peer-to-peer system of several nodes communicate with each other via message passing. Nodes may be exposed to crashes and the network to partitioning. Furthermore, some of the nodes of the network may also exhibit malicious behavior, that is, we consider Byzantine faults. Nodes are assumed not to know the identity of Byzantine nodes at the start of execution, nor to what extent they control the network.
%As related work has largely focused on applications within financial services, this project may provide insight into novel challenges related to consensus in SCM blockchain systems. Furthermore, the project aims to provide experimental data, comparing candidate consensus algorithms in a realistic setting, employing the industry adopted blockchain platform Hyperledger Sawtooth. Combined, this is aimed towards providing blockchain designers with sufficient information to make well-informed decisions regarding their choice of consensus mechanisms, given the aforementioned SCM setting. 


%This motivation leads to the following research questions:

%\todo{Research questions mentioned trice, remove?}
%\textbf{RQ1:} What consensus models are able to provide integrity in an environment with limited network throughput?

%\textbf{RQ2:} What consensus models are able to provide security in an environment with limited network throughput?


%\subsection{Contributions}

% provide insight into how state of the art consensus algorithms will provide high transaction throughput, security and decentralization, in an enterprise setting, with a system exposed to varying/high network delay.

% Focusing specifically on usage within SCM can uncover novel challenges specific to the domain. This can support future work

%The expected contribution of this research is to provide insight into how state of the art consensus algorithms will provide integrity and security in an enterprise setting with a system exposed to varying network throughput, emphasizing good performance. This will be in form of an analysis of current state of the art consensus algorithms and their performance characteristics, as well as experimental data, deploying a set of promising candidate algorithms in a realistic setting and reviewing their relative performance. The existing literature has primarily focused on blockchain usage within financial services, assuming a relative stable network. The project will therefore provide a unique perspective. 

%The research project is furthermore intended to contribute in creating new blockchain platforms, better facilitating SCM blockchain systems. In particular, by specifically focusing on usage within SCM, the project may uncover novel challenges specific to the domain, enabling future work. 


%\subsection{Research Methods}

%The project will start with an initial systematic mapping study of consensus algorithms, focusing on how each algorithm ensures integrity and security, while also providing good performance, in an environment with limited network throughput. The study will consist of both white and gray literature, reflecting both the state of academia, as well as industry. This will provide insight into current state of the art, as well as providing valuable input for the project's overall direction. By reviewing existing literature, the project's conceptual framework and research questions can be further refined. 

%Following this, a set of candidate consensus algorithms will be selected. This will be based on the information gathered throughout the systematic mapping study. These algorithms will then be implemented for a relevant industry-tested blockchain platform, Hyperledger Sawtooth \citep{Sawtooth}. This will allow for an experimental study of consensus algorithms, comparing candidate algorithms among themselves, as well as Hyperledger Sawtooth's existing implementations. This is essential, providing empirical evidence supporting any further recommendations of consensus algorithms in networks with unstable network throughput. 

%Based on observations from the experimental studies, analysis of the consensus algorithms' performance characteristics can be provided. This is then aimed to provide a foundation for recommendations regarding choice of consensus mechanisms in the described SCM setting.


% Removed: This picture is not necessary
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.75\textwidth]{graphics/research_methods_edit.png}
%\end{figure}



%\subsection{Participants}

%The majority of the work will be conducted by Henrik Knudsen, as part of his specialization project and master thesis. Supervision of the project will be provided by Associate Professor Jingyue Li,  Researcher Peter Halland Haro and PhD Candidate Jakob Notland. Li will act as the project's main supervisor, monitoring progress and providing guidance. Haro and Notland will acts as co-supervisors, assisting in selecting the project's related literature, as well as providing feedback and technical advice. Furthermore, Haro will provide assistance regarding setting up a test environment, to be used during the experimental study.

%Knudsen will primarily conduct the initial systematic mapping study. Li, Haro and Notland will provide assistance regarding screening papers for the study. Knudsen will then be responsible for implementing, testing and evaluating candidate consensus algorithms, with guidance from Li, Haro and Notland. 



%\subsection{Research Paradigm}

% Positivism, if doing experiments
% Researchers will systematically investigate current state of the art consensus algorithms, emphasizing formal proofs, as well as statistical data supporting performance claims. Furthermore, the researchers will carry out experimental studies, gathering empirical evidence supporting  these claims. Based on this, the research is therefore deemed to fall within the positivism paradigm. 

%\subsection{Final deliverables}

%The research project has several deliverables. The results of the initial systematic mapping study will constitute a project report. Furthermore, the study will be submitted as a paper, for the 3rd IEEE International Conference on Blockchain and Cryptocurrency Spring 2021. Combined with the mapping study, the experimental study and observations will constitute the master thesis.

==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/results.tex <==
\section{Research Results}
\label{sec:study_results}
We first classified the 25 consensus algorithms identified from the literature into five categories, namely, Nakamato, Byzantine Fault Tolerant (BFT), Federated Byzantine Agreement (FBA), Hybrid, and Crash Tolerant, based on their core principles. Then, we analyzed 1) whether the algorithm provides sufficient performance in this specific application scenario with limited network throughput; 2) whether the algorithms provide integrity in the application scenario, as of RQ1; 3) to what extent the algorithms provides security in this application scenario, as of RQ2. The findings related to the performance metrics are summarized in Table \ref{tab:app_classification}. The answers to RQ1 and RQ2 are summarized in Table \ref{tab:discussion_summary}.

\subsection{Performance}

\textbf{Nakamoto style} consensus algorithms usually provide consensus in a single communication step, except PoA. They all operate with linear complexity as well as requiring an honest majority. The timing assumption is synchronous, which is challenging with low network throughput. With probabilistic finality, there is also a great chance of forking given our SCM application scenario.

\textbf{BFT style} consensus algorithms usually provide consensus in a three communication step process, with quadratic communication complexity. Delegated BFT, Mixed BFT, and Linear-BFT can achieve linear communication complexity through partitioning the network. Delegated BFT and Mixed BFT delegate consensus to a subset of the nodes in the network. Linear-BFT reduces the number of messages sent per node by using an expander graph. This, however, comes at the cost of either significantly increased centralization or potentially higher consensus latency. BFT style consensus algorithms all provide deterministic finality, which may be of major benefit, providing low confirmation latency for transactions. In the enterprise setting, this can be a deciding factor. These consensus algorithms can typically withstand a maximum of $\frac{1}{3}$ Byzantine nodes, posing a significantly weaker resistance than the honest majority threshold provided by Nakamoto style consensus algorithms. Linear-BFT emerges as a promising innovation, providing the optimal threshold of $\frac{1}{2}$ Byzantine nodes, while also having amortized optimal communication complexity of $\Theta(n)$. 

%FDA
\textbf{FBA style} consensus algorithms do not provide any guarantees to the number of consensus steps involved in agreeing upon a set of transactions. As nodes only communicate within their respective quorum slice, communication complexity depends on each node's quorum slice's size. In Ripple, Unique Node Lists (UNL) need to overlap 90\% across the network to ensure security, making communication complexity $\Theta(n^2)$. In SCP, nodes are free to pick their quorum slices based on their own reasoning (e.g., reputation, wealth, brand). In an optimistic setting, where the size of quorum slices is constant, SCP's communication complexity is $\Theta(n)$. SCP furthermore provides optimal resilience towards Byzantine nodes in the federated setting, only requiring that nodes' quorum slices intersect honestly. RPCA makes an assumption of a maximum of 20\% Byzantine nodes for a given UNL list. As FBA agreement builds upon nodes' quorum slices intersecting, consensus relies on that not all these interconnections are faulty. If these critical nodes suffer from low network throughput, this could hamper the speed and throughput in which the network can process transactions. In particular, if they cannot respond for a long time, transaction throughput may halt.

%Hybrid
\textbf{Hybrid style} consensus algorithms typically provide consensus in linear communication complexity using a three-step BFT style process to reach consensus, while using mechanisms from Nakamoto style consensus algorithms for leader election. This scheme allows for immediate finality, which enables consensus algorithms to work in a permissionless setting. The consensus algorithms can scale better than standard Nakamoto consensus algorithms with the cost of reduced Byzantine fault tolerance.

\textbf{Crash tolerant style} consensus algorithms, i.e., Raft, provide consensus in a single communication step, with the optimal communication complexity of $\Theta(n)$. It also provides deterministic finality. The main caveat related to crash tolerant consensus algorithms is that they cannot tolerate Byzantine faults. Disregarding Byzantine faults, Raft tolerates up to 50\% crashed nodes. Raft's communication pattern is completely leader-centered. During normal operation, the leader continuously broadcasts messages to the rest of the network, while follower nodes only respond to the messages they receive. Therefore, the leader node must have sufficient network throughput and computational resources for the leader not to become a bottleneck in terms of performance.

\begin{table*}[t]
 \centering
\begin{tabular}{p{3cm}llllrl}
    Name & Ref & Latency & Complexity & Timing assumptions & BFT & Finality \\\hline
     \multicolumn{7}{l}{\textbf{Nakamoto style consensus algorithms}} \\\hline
     PoW & \citep{Nakamoto_Bitcoin_POW} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \% & Probabilistic\\
     PoS & \citep{RN64} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \% & Probabilistic\\%, Nothing at stake \\
     DPoS & \citep{DPOS_Larimer} & 1 RTT & $\Theta(n)$ & Synchronous   & 50 \%& Probabilistic \\%, High centralization \\
     DDPoS & \citep{DDPOS_White_IEEE} & 3 RTT & $\Theta(n^2)$ & Synchronous &  50 \% & Probabilistic\\
     PoAuth & \citep{RN66} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \%& Probabilistic \\
     PoET & \citep{POET_SPEC} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \% & Probabilistic\\
     PoTS & \citep{RN67} &  1 RTT & $\Theta(n)$ &  Synchronous& 50 \% & Probabilistic\\
     PoR & \citep{RN68} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \% & Probabilistic\\
     PoB & \citep{RN69} & 1 RTT & $\Theta(n)$ & Synchronous & 50 \% & Probabilistic \\
     PoC & \citep{RN70} & 1 RTT & $\Theta(n)$ &  Synchronous & 50 \% & Probabilistic\\
     PoI & \citep{NEM_POI} & 1 RTT & $\Theta(n)$ &  Synchronous & 50 \% & Probabilistic\\
     PoA &  \citep{POA} & 3 RTT & $\Theta(n)$ &  Synchronous & 50 \% & Probabilistic \\\hline
     \multicolumn{7}{l}{\textbf{BFT style consensus algorithms}} \\\hline
     Linear-BFT & \citep{RN36} & 6 RTT & $\Theta(n)$ & Synchronous & 50 \% & Immediate \\
     PBFT & \citep{PBFT_MIT} & 3 RTT & $\Theta(n^2)$ &  Partial Synchronous & 33 \% & Immediate\\
     IBFT & \citep{RN37} & 3 RTT & $\Theta(n^2)$ & Partial Synchronous & 33 \% & Immediate\\
     Delegated BFT & \citep{RN71} & 3 RTT & $\Theta(n)$ & Partial Synchronous  & 33 \%  & Immediate\\ %High Centralization \\
     BFT - SMART &  \citep{BFT_SMART} & 3 RTT & $\Theta(n^2)$ & Partial Synchronous  & 33  \% & Immediate \\
    T-PBFT & \citep{RN34} & 3 RTT & $\Theta(n^2)$ & Partial Synchronous  & 33 \% & Immediate\\ %, High centralization \\
      MBFT & \citep{RN33} & N/A & $\Theta(n)$ & Partial Synchronous & 33 \% & Immediate\\
    Honey-BadgerBFT & \citep{RN42} & 6 RTT & $\Theta(n^2)$ & Asynchronous & 33 \% & Immediate\\\hline
    
      \multicolumn{7}{l}{\textbf{Federated Byzantine Agreement consensus algorithms}} \\\hline
     RPCA & \citep{RIPPLE_ANALYSIS} & N/A & $\Theta(n^2)$ &  Partial Synchronous  & 20 \% & Immediate \\
     SCP & \citep{SCP} & N/A & $\Theta(n)$ & Partial Synchronous & N/A & Immediate \\\hline
     \multicolumn{7}{l}{\textbf{Hybrid consensus algorithms}} \\\hline
     BFT-based POW & \citep{RN73} & 3 RTT & $\Theta(n)$ &  Partial Synchronous & 33 \% & Immediate \\ % High  centralization \\
     BFT-based POS & \citep{RN72} & 3 RTT & $\Theta(n)$ &  Partial Synchronous & 33 \%  & Immediate\\\hline % High  centralization \\
     \multicolumn{7}{l}{\textbf{Crash Tolerant consensus algorithms}} \\\hline
     Raft & \citep{RAFT} & 1 RTT & $\Theta(n)$ &  Partial Synchronous & 0 \% & Immediate \\
\end{tabular}
\caption{Consensus algorithm classification}
    \label{tab:app_classification}
\end{table*}

\begin{table*}[h]
    \centering
    \begin{threeparttable}
    \begin{tabular}{p{4cm}lllll}
    
         \multicolumn{6}{p{14cm}}{\rule{0pt}{6ex}\textbf{RQ1: What consensus models are able to provide integrity in an environment with limited network throughput?}}\\\hline
         \textbf{Consensus algorithms} & Nakamoto & BFT & FBA & Hybrid & Crash Tolerant \\\hline
         Integrity in asynchronous system & - & ! & + & + & + \\
         \multicolumn{6}{p{14cm}}{\rule{0pt}{6ex}\textbf{RQ2: What consensus models are able to provide security in an environment with limited network throughput?}}\\\hline
         \textbf{Consensus algorithms} & Nakamoto & BFT & FBA & Hybrid & Crash Tolerant \\\hline
         Double spend attacks & - & + & + & + & ! \\
         Balance attacks & - & + & + & + & + \\
         Long-Range attacks & ! & + & + & + & + \\
         P + Epsilon attacks & ! & + & + & + & + \\
         DDOS attacks & + & - & ! & - & - \\
         BGP attacks & - & - & ! & - & - \\
    \end{tabular}
    \bigskip
    \begin{flushleft}
        \begin{tablenotes}
            \item[+] Strong guarantees
            \item[-] Lacking guarantees
            \item[!] Depending on the specifics of the consensus algorithm or the configuration of the blockchain system
            %\item[*] Linear-BFT provides $\Theta{(n)}$ communication complexity.
        \end{tablenotes}
    \end{flushleft}
    \caption{Summary of consensus algorithms in relation to performance metrics, RQ1 and RQ2. }
    \label{tab:discussion_summary}
    \end{threeparttable}
\end{table*}


\subsection{Integrity}
Limited network throughput may cause increased asynchrony within a blockchain system. This makes it infeasible to make assumptions regarding the ordering or timing of messages being sent. As such, consensus algorithms relying on synchronous network for correctness cannot provide integrity in the relevant setting.

\textbf{Nakamoto style} consensus algorithms are unfit for the setting \citep{RN45}. 

\textbf{BFT style} consensus algorithms may work depending on their timing assumptions. Linear-BFT specifically assumes synchronous network and therefore cannot guarantee integrity either. BFT consensus algorithms assuming a partial synchronous or asynchronous network will still provide integrity in such an asynchronous network. It is important to point out that while many BFT style consensus algorithms can provide integrity during times of asynchrony, these same algorithms cannot provide liveness at the same time, as a result of the FLP impossibility \citep{RN40}. The network needs to stabilize before transactions can be continued to be processed. In light of this, the Honey-BadgerBFT consensus algorithm differentiates itself, as it makes no assumptions regarding the network's synchrony. As Honey-BadgerBFT functions purely asynchronously, it may avoid the standstill of asynchrony or performance impact of a larger message delay $\Delta$. In particular, \citep{RN42} points out that there will always be an inherent trade-off related to such synchrony assumptions. If the $\Delta$ parameter value is too low, the system will not provide progress. If the $\Delta$ parameter value is too high, it will not fully take advantage of the network's bandwidth. The authors propose Honey-BadgerBFT as a candidate for consortium blockchain systems, emphasizing its benefits of robustness and high transaction throughput, despite being an asynchronous system.

\textbf{FBA style} consensus algorithms, i.e., RPCA and SCP, assume a partially synchronous network and can provide integrity even in periods of asynchrony. However, they require messages to be bounded by some upper bound message delay $\Delta$ to provide forward progress. 

\textbf{Hybrid style} consensus algorithms Byzcoin and Tendermint make synchronization assumptions equal to that of partial synchrony. In times of asynchrony, consensus algorithms can preserve integrity. Conversely, the consensus algorithms' transaction throughput may suffer significantly during these events, similar to that of BFT style consensus algorithms.

\textbf{Crash tolerant style} consensus algorithm relies on synchronization assumptions similar to that of BFT style consensus algorithms. In particular, Raft assumes a known broadcasting latency, which is then used to determine an election timeout interval. The algorithm can ensure integrity, even in periods of asynchrony, despite the message delay exceeding the assumed bound. However, it will not be able to provide any forward progress in such events. There will be a continuous re-election process until the network stabilizes. This may be problematic in terms of a network with high communication latency and poor network throughput. 

\subsection{Security}

\textbf{Nakamoto style} consensus algorithms are targets of a multitude of attacks. Sufficient delay of messages caused by the asynchrony of the network may enable double spend and balance attacks. Furthermore, the Nakamoto style consensus algorithms may be vulnerable to P + Epsilon attacks, depending on the blockchain system's incentivization mechanisms. In contrast to many other types of consensus schemes, which are centered around a stable leader, Nakamoto style consensus algorithms elect leaders non-deterministically on a block-to-block basis, which makes DDOS attacks infeasible in most practical settings. Conversely, the consensus algorithms may, however, be vulnerable to BGP attacks. In particular, \citep{RN53} has shown the feasibility of utilizing routing attacks against Bitcoin's PoW scheme.

%DDOS attacks may be particularly relevant, given an environment affected by varying network throughput. In relation to leader-centered BFT, Hybrid and Crash tolerant consensus algorithms, adversaries may target the leader with continuous DDOS attacks, halting the forward progress of the blockchain system. A variation of this attach may also be applicable to Federated Byzantine Agreement consensus algorithms, in that well-connected nodes may be targeted, creating divergence within the network. An adversary may also target arbitrary nodes within the network, in an attempt to break the fault tolerance threshold of the consensus algorithm. The feasibility of this depends on the size of the network, current number of faulty nodes, as well as the adversary's computational resources. It is deemed that this would be easier to do against consensus algorithms with lower fault tolerance. For instance, Nakamoto consensus algorithms, providing 50\% fault tolerance, are more robust against such attacks than most BFT style consensus algorithms, providing 33\% fault tolerance.

%BGP attacks are deemed generally applicable to most consensus algorithms. By gaining control of parts of the routing infrastructure used within the network, adversary may partition the network and delay messages. This may be sufficient to enable double spend and balance attacks against Nakamoto Consensus algorithms, further exasperated by the already existing asynchrony of the network, caused by limited network throughput. Routing attacks may also target BFT, Hybrid and Crash tolerant consensus algorithms, either by targeting the traffic of the leader, hampering liveness, or by targeting arbitrary nodes, attempting to break the consensus algorithm's fault tolerance threshold. Whether routing attacks are applicable towards Federated Byzantine Agreement consensus algorithms may depend on the overall topology of the network; if an adversary is able to target a particularly well-connected node, then this may be sufficient to create divergence within the network, hindering the achievement of consensus.

\textbf{BFT style} consensus algorithms usually have an increased susceptibility towards DDOS attacks, compared to Nakamoto style consensus. Specifically, when sufficiently powerful adversaries have insight into which of the network's nodes is the leader for a given election term or view, they could impair the system's liveness by overloading the leader with incoming traffic. This is exasperated in our SCM setting with low network throughput. As many BFT style consensus algorithms rely on a stable leader for progress, in the worst case, this could lead to a continuous view change, grinding transaction throughput to a halt. The Honey-BadgerBFT consensus algorithm once again differentiates itself from the other BFT style consensus algorithms in that it is leaderless. Therefore, the Honey-BadgerBFT consensus algorithm does not suffer from the aforementioned susceptibility towards DDOS attacks. DDOS attacks could also potentially target non-leader nodes in an attempt to increase the number of faulty nodes. As most BFT style consensus algorithms require a supermajority of honest nodes to ensure the system's integrity, a sufficiently powerful adversary could target honest nodes and break the Byzantine Fault Tolerance threshold. Whether this would be feasible in a practical setting depends on the size of the network, the current number of Byzantine nodes, as well as the adversaries' combined computational resources. Linear-BFT, which only requires a majority of honest nodes to ensure integrity, may be better suited to defend against this kind of attack. BFT style consensus algorithms could also be vulnerable to BGP attacks. When an adversary gains control of routing mechanisms used within the system, they could potentially partition the network or delay communication between nodes. Targeting the leader could hamper the liveness of the system. When the adversaries have access to an especially central router within the communication system, they could isolate larger groups of participants. Like a DDOS attack, this could allow adversaries to break the Byzantine Fault Tolerance threshold, invalidating any guarantees about the system's integrity.  

\textbf{FBA style} consensus algorithms avoid some of the pitfalls related to BFT style consensus. In particular, as RPCA and SCP are leaderless, there is no vulnerability related to a leader being targeted by a DDOS attack, stopping the system from achieving progress. There is, however, a new potential attack vector related to splitting the network. Going back to the important role in which intersecting nodes play in federated Byzantine agreement, a sufficiently powerful adversary could perform DDOS attacks targeting well-connected nodes. Such an attack could partition the network, isolating nodes, making consensus in the original network unachievable, and hindering transaction throughput. FBA style consensus algorithms could be vulnerable to the BGP attack. Similar to that of a targeted DDOS attack against a well-connected node, if an adversary gains control of a central router within the communication network, they could partition the network, creating divergence. In terms of RPCA, where the 90\% UNL overlap makes divergence attacks unlikely, attackers might rather try to break the Byzantine Fault Tolerance threshold of 20\%. As for SCP, allowing users to communicate only with nodes selectively they specifically trust, any form of substantial routing attack may break the network, depending on the size of each user's node list.

\textbf{Hybrid style} consensus algorithms have an increased susceptibility to DDOS attacks due to the transition from Nakamoto style consensus to a hybrid approach. Like BFT style consensus algorithms, the hybrid approach is leader-centered and needs to maintain a stable leader to provide high performance. Combined with limited network throughput, this may further hinder transaction throughput. DDOS attacks might also target non-leader nodes of the network. As inclusion in the inner consensus group is the core of Nakamoto style consensus mechanisms, attacking arbitrary nodes would require most nodes to become faulty before the Byzantine Fault Tolerance threshold would break. If the adversary instead chooses to target the inner consensus group, the threshold is reduced to only 33\% of the consensus group itself, and as such, should be significantly more feasible. Furthermore, hybrid style consensus algorithms are vulnerable to BGP attacks. Combining Nakamoto and BFT style consensus mechanisms, Hybrid style consensus algorithms inherit both groups' vulnerabilities related to BGP.

\textbf{Crash tolerant style} consensus algorithm suffers from the same DDOS susceptibility as BFT style consensus algorithms. The consensus algorithm needs to maintain a stable leader to provide liveness, and such, continuous DDOS attacks targeting leaders can hamper transaction throughput. This may be further exasperated by nodes having limited network throughput. Similar to BFT style consensus algorithms, a DDOS attack may also be used against arbitrary network nodes. In Raft's case, to break the Crash Tolerance threshold, a total of 50\% of the network nodes must become faulty. Thus, unless the network is volatile and at some points contains a lot of faulty nodes, such an attack would be less practical than targeting the leader directly. Finally, Raft is also vulnerable to BGP attacks. An adversary initiating a routing attack against the network leader would be able to completely halt transaction throughput, hindering any broadcasts from reaching the follower nodes. Furthermore, given sufficient power, the adversary could partition the network, attempting to break the Crash Tolerance threshold of 50\%, enabling double spends.




==> Consensus_systematic_mapping_IEEE_prepared(1)/sections/scenario.tex <==
%\section{Application scenario}
%\label{sec:app_scenario}
% Section will give insight into application scenario of blockchain technology and the specific scenario which we focus on in this paper.
%This section describes the specific application scenario we consider in our research; enterprise blockchain systems used within SCM, with low network throughput. Additionally, the limitations of the research are then described, based on the context of the application scenario.
%\subsection{Scenario}
%In this paper, we specifically envision an enterprise, permissioned blockchain system. The participants of the network are comparable to that of independent organizations, utilizing the blockchain system in a cooperative manner. 
We assume an authenticated setting, in which each node $N_i$ have established a cryptographic encryption key $Ek_{i,j}$ with their respective \textit{neighbors} $N_j \in N$ , before the execution of a round of consensus. Here neighbors refer to any node in which $N_i$ either need to send or receive messages from, in order to carry out a round of the consensus algorithm. Having established such an encryption key, a message passing between two nodes is assumed to be comparable to a single round-trip time, i.e. 1 RTT. 

A consensus algorithm's communication complexity is measured in terms of the number of bits sent, related to the number of nodes $n$ in the network. A round of consensus involves both reaching an agreement, as well as propagating necessary data within the network in order for all nodes $N_i \in N$ to be able to commit the decided block to their local ledger. Following this understanding, an optimal consensus algorithm in terms of communication complexity involves $\Omega(n)$ bits being sent each round.

Network nodes are assumed to be heterogeneous. In particular, nodes may have different computational and memory resources, use different communication protocols among each other, and have varying geographical distance between each other, contributing to the network latency. Furthermore, the network is assumed to possibly span a large geographical area, in which nodes may have widely varying network latency among each other. This latency may also change over time, e.g. a node corresponding to a vessel transporting goods may move closer to one of its neighbors, thus reducing the network latency among them. 

A particular constraint of the network are periods of limited network throughput. Specifically, the network's nodes $N$ are assumed to be either stable, denoted $N_s$, or unstable, denoted $N_u$. Unstable nodes are expected to experience periods of poor or no network connection, in contrast to stable nodes, which are expected to exhibit a consistent connection across consensus rounds. As an illustrating example, a stable node could correspond to an office building in a metropolitan area, having access to a high speed WLAN, while an unstable node could correspond to a vessel traveling international waters, where as access to the internet may vary during the vessel's voyage. 

\subsection{Limitations}

% permissioned - need way to govern network. Assume authenticated.

The scenario focus solely on a permissioned setting. Specifically, there is some administrative structure which governs who are allowed to participate in the network. Furthermore, we assume an authenticated setting. This limits the research in terms of public blockchain systems. In particular, the need for Sybil attack resistance is relaxed, as all participants of the network are authenticated and approved by the system. 

% low network throughput - 

A differentiating factor of the scenario is that the system is significantly affected by low network throughput. This increases the effect which communication related costs have on metrics such as transaction throughput. Furthermore, since a subset of the nodes may experience poor network throughput, the system may be especially asynchronous, compared to other scenarios. This limits the research to systems affected by such constraints. In particular, blockchain systems with stable network throughput may emphasize other considerations in terms of their consensus mechanisms, as communication costs become less significant.

% high latency - geograpically distributed
Finally, as the nodes of the network are distributed over a large geographical area, some nodes may experience high network latency in communicating with other nodes. This may significantly affect consensus mechanisms which rely on timing assumptions related to the network. The research is therefore limited to that of networks of scale; if a system's nodes are closer in distance, latency related costs may be negligible. 




==> sections/background.tex <==
\section{Background}

%This section provides necessary background information related to the research. In particular, a brief overview of blockchain technology is provided, highlighting its architecture and key characteristics. Then, terminology and important results related to consensus mechanisms are explained. Finally, important security considerations regarding blockchain systems are discussed, based on the reviews of \citet{RN17} and \citet{RN30}. 


%\subsection{Blockchain technology}

%This section provides a brief overview of blockchain technology; what constitutes a blockchain, key characteristics and the role in which consensus algorithms play in blockchain technology. 



%A blockchain is a specific form of Distributed Ledger Technology (DLT) \citep{RN59}, allowing for the geographical replication, sharing and synchronization of data between peers. Blockchain differentiates itself from other types of DLTs, in that the data it contains are organized as a sequence of blocks, as seen in figure \ref{fig:background_chain}. Each block contains a block header, containing header information, as well as some data, e.g. a list of financial transactions. In particular, the block header contains the hash of the block's parent block. The hash acts as an unique identifier of the parent block. Thus,  a sequential linkage of blocks are created, i.e. a chain, from the most recent block, all they way back to the chain's starting block, denoted the genesis block. 


%\begin{figure}[h]
%    \centering
%    \hspace*{-0.6cm}
%    \includegraphics[width=0.55\textwidth]{graphics/blocks.png}
%    \caption{Visualization of linked blocks, constituting a blockchain. Reprinted from \citet{RN58}. }
%    \label{fig:background_chain}
%\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.5\textwidth]{graphics/block.png}
%    \caption{Visualization of single block, containing header information, as well as data in the form of transactions. Reprinted from \citet{RN58}. }
%    \label{fig:background_block}
%\end{figure}

%A representative blockchain block is shown in figure \ref{fig:background_block}, similar to that used in the cryptocurrency Bitcoin \citep{Nakamoto_Bitcoin_POW}. In addition to the parent block reference, the block header may also contain the following information\footnote{The nBits and Nonce fields are specific to that of blockchain system utilizing a Nakamoto style consensus algorithm, popularized by Bitcoin \citep{Nakamoto_Bitcoin_POW}. In blockchain systems utilizing other types of consensus algorithms, these may be omitted.} \citep{RN58}: \begin{itemize}
    %\item \textbf{Block Version}: The specific version of the blockchain system used when generating the block. Used to keep track of protocol changes.
    %\item \textbf{Merkle Tree Root Hash}: A hash tree of the transactions contained in the block. Ensures the integrity of the transactions stored.  
    %\item \textbf{Timestamp}: Block generation time. Given in seconds, universal time, from January 1, 1970. 
    %\item \textbf{nBits}: Target threshold for a valid block hash. Corresponds to the difficulty level of the blockchain system used when the block was generated. 
    %\item \textbf{Nonce}: The hash value used to solve the target threshold, allowing the generation of the block. 
%\end{itemize}

%Key characteristics of blockchain technology is its ability to provide a high degree of security and robustness. By replicating the data stored within the blockchain across multiple nodes, the system may provide higher availability than that of a centralized system. Furthermore, by the use of strong cryptographic mechanism, such as digital signature and cryptographic hash functions, the validity of the data committed to the blockchain may be verified. This may be particularly important in a financial setting, e.g. asserting that the details of the transaction is correct and that the parties involved are who they claim to be.

%In order to ensure the integrity of the data stored within each respective block in the blockchain, a cryptographic mechanism called a \textit{Merkle Tree} may be utilized \citep{RN60}. As shown in figure \ref{fig:background_merkle}, the leaves of the merkle tree correspond to the data stored in the blockchain, e.g. a set of transactions. A cryptographic hash function is then  used to transform the data into a single root hash value, forming a tree structure. Given the avalanche effect of cryptographic hash functions \citep{RN61}, this allows for cost effective ways of detecting damage or adversarial tampering with the data stored in the blockchain. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.4\textwidth]{graphics/merkle_tree.png}
%    \caption{Visualization of a merkle tree used to ensure the integrity of transactions stored in blockchain. Only the root hash value is kept in block header. Reprinted from \citet{Nakamoto_Bitcoin_POW}. }
%    \label{fig:background_merkle}
%\end{figure}

%To ensure consistency of data shared between participants in the blockchain system, a consensus algorithm is used \citep{RN58}. A consensus algorithm provide a means for participants to reach agreement about a set of values, in a decentralized fashion, without necessitating trust between the participants. The consensus algorithm need to be able to protect the system against adversarial attacks, such as tampering with data, delaying of communication or other malicious behavior.

%Popularized by Bitcoin, Proof of work is a commonly used consensus algorithm, based around participants solving a cryptographic puzzle; when generating a new block, the block header need to be smaller than certain difficulty value. By incrementing the nonce value in the block header, the participants, often denoted miners, may do computational work in order to be allowed to generate the next block, often in return of some reward. Given the the use of a cryptographically strong hash function, this is comparable to a lottery and buying tickets; the amount of computational work a participant puts into solving the puzzle corresponds directly to their chance of winning the next block and reward. Which participants who get to generate the next block is therefore randomized. When a participant finds a solution to the puzzle, they generate the block, include the solution nonce value in the block header, and broadcast it to the rest of the network. The remaining participants verify the validity of the block, and if correct, adds it to their local chain. Given that a majority of the computational power of the network is owned by honest participants, the consensus algorithm can provide strong security guarantees in many types of blockchain networks.

% Meta information removed - the information in not necessary, and I dont need to spend time figuring out why the ref is bugged.
%(for further information on consensus in blockchain, see section \ref{subsec:background_consensus} and section \ref{sec:sota_consensus}). 

%Originating from the success of the cryptocurrency Bitcoin, a multitude of new use cases have been proposed for blockchain technology in recent years. In particular, it has been promoted as a way for independent organizations to share data, in a transparent and secure manner. This has lead to a distinction between permissionless and permissioned blockchain systems: \begin{itemize}
%    \item \textbf{Permissionless blockchain}: Anyone may access the blockchain system.
%    \item \textbf{Permissioned blockchain}: Access to the blockchain is regulated. Only approved entities may participate in teh blockchain system.
%\end{itemize}
%In particular, Bitcoin is an example of a permissionless blockchain system, allowing anyone to trade cryptocurrency. Permissioned blockchain systems may only involve a select few participants, e.g. a partnership between medical institutions to share patient data. Utilizing a permissioned blockchain system may have several benefits, in that access is constrained to only certain participants, providing some level of inherent data confidentiality. Furthermore, as participants are authenticated, the blockchain systems may use different consensus algorithms than that of a permissionless system, potentially offering better performance, energy efficiency or other benefits. 



%\subsection{Consensus mechanisms} \label{subsec:background_consensus}

%This section describes core concepts and terminology related to consensus in distributed systems and consensus algorithms. 

%\subsubsection{Safety and Liveness}

%Central to discussing the integrity and security of consensus mechanisms are the properties of \textit{safety} and \textit{liveness}, established by \citet{RN48}. \textit{Safety} means that incorrect operations cannot happen during execution. \textit{Liveness} mean that correct operations will eventually be executed by the system. Safety is comparable to the correctness of the consensus algorithm. In particular, according to the assumptions made by the consensus model, there is no sequence of events in which the system can enter an erroneous state. As an illustrating example, despite the presence of a adversarial environment, the Nakamoto consensus scheme is able to ensure eventual consistency within the Bitcoin network, given that the assumption of an honest majority within the network holds. Conversely, liveness is comparable to the consensus algorithm's ability to make forward progress. While it is essential that the algorithm is correct, if the algorithm cannot provide liveness, it cannot be effectively utilized in a practical setting. As another illustrating example, despite interference from adversarial parties, honest actors participating in the Nakamoto consensus are eventually able to agree upon a set of transactions, given an honest majority within the network. 

%\subsubsection{Fault tolerance}

%It is a desired quality of consensus algorithms that they are able to tolerate faulty nodes. In particular, for the system to gain  robustness from being distributed across multiple nodes, it must be able to reach consensus despite a subset of the nodes having failed. 

%There are numerous types of faults which may be considered in relation to distributed computing systems. In the context of systems affected by an adversarial environment, such as a permissionless blockchain system, one often consider \textit{Byzantine fault tolerance}. A Byzantine fault is a complex type of fault, in which there is imperfect information related to whether a certain node has failed. Derived from the Byzantine General's problem \citep{RN49}, it depicts a situation in which a node may inconsistently appear faulty from the perspective of other nodes of the network; a node A may seem unresponsive to node B, while it may at the same time respond to messages from node C and therefore seem correct from their perspective. Byzantine faults oftentimes is used to model arbitrary or malicious behavior within the network, in which an adversary may choose to not follow protocol, and thus selectively send information, neglect to respond to messages etc. Byzantine fault tolerance is a measure to which degree a distributed system can withstand Byzantine faults within the network.

%Another type of fault tolerance to consider is \textit{crash tolerance} \citep{RN50}. In this simplified model, one consider non-Byzantine types of faults, in that nodes may crash, but may not show arbitrary behavior. While corresponding to a weaker adversarial model, it is representative for many practical settings, specifically towards to that of a private blockchain system. 

%\subsubsection{CAP Theorem}

%A well known limitation towards distributed systems is the CAP theorem \citep{CAP}. The theorem asserts that it is impossible for a distributed system to simultaneously provide the following qualities: \begin{itemize}
%    \item \textbf{Consistency}: All requests received by the system are executed atomically; as if the system was a single entity. 
%    \item \textbf{Availability}: All requests receive non-error responses. 
%    \item \textbf{Partition Tolerance}: The system continues to operate despite an arbitrary number of messages being lost between network nodes.  
%\end{itemize} 

%\citet{CAP} goes on to prove that systems are able to provide 2/3 out of the qualities, in particular AP, CA or CP. In practical systems, where network nodes are geographically distributed and network partitioning is a definite possibility (e.g. communication is done over the internet), the choice is oftentimes narrowed down to AP or CP. Specifically, in the case of network partitioning, a choice must be made regarding to provide either availability or consistency.

%Consensus mechanisms used within blockchain systems must adhere to the CAP theorem \citep{RN47}. In particular, in the case of network partitioning, the system must either make compromises towards consistency or availability. Examples of this can be seen in systems utilizing Nakamoto style consensus, in which forks may happen, creating periods of inconsistency within the network. The system therefore sacrifices strong consistency in favor of availability. In contrast to this, systems using deterministic BFT style consensus algorithms cannot fork, and such opt for strong consistency, sacrificing availability in the event of network partitioning. 

%This can further be related to a consensus algorithm's transaction finality; the algorithm's guarantee that committed transactions cannot be reversed. Consensus algorithms providing probabilistic finality, e.g. Nakamoto style consensus, favor availability over strong consistency. Consensus algorithms providing immediate finality, e.g. BFT style consensus, need strong consistency to enforce this, thus sacrificing the system's availability during network partitioning.     

\subsubsection{FLP Impossibility}
\label{subsub:FLP}

% result

An important result within distributive systems is the so called \textit{FLP Impossibility} result. \citet*{RN40} prove that one cannot achieve deterministic consensus in an asynchronous, distributed system with at least a faulty node. This has major implications on consensus in blockchain systems, as communication between peers are over the internet in most practical settings, which is inherently asynchronous, and one oftentimes desire some non-zero level of fault tolerance. 

\citet{RN40} reach this conclusion by proving that in the fully asynchronous setting, utilizing a deterministic consensus algorithm, there exist some configuration of nodes $C$, in which the system cannot reach an decision, given at least a faulty node. In specific, given a network of N nodes, all with some input value $x_i \in \{0,1\}$, with the goal of agreeing upon a common output value $y \in \{0,1\}$, there exist a configuration of input values among the nodes in which $y$ may be undecided\footnote{\citet{RN40} scenario is specifically related to that of Binary Byzantine Agreement, but can be extended to consensus about non-binary values. }. 

The authors prove this by making the observation that there must exist two configurations $C_0$ and $C_1$ which lead the consensus algorithm to agree on different values, but which also only differ in the input value of a single node $n$. Such, the result of the consensus round depends on the value contributed by the node $n$. Without loss of generality, assume that $C_0$ gives an output $y = 0$ and $C_1$ gives an output of $y = 1$.  Should $n$ be faulty (i.e. it does not contribute its value during the consensus round), $C_0$ or $C_1$ cannot be differentiated, and thus should decide upon the same value, as the consensus algorithm is deterministic. If the value they decide upon is $y = 1$, then $C_0$ is indecisive; the configuration may lead to either values being decided upon. The same holds for $C_1$ in the case of $y = 0$. Therefore, there exist some configuration $C$ in which one cannot deterministically decide upon a value.

The authors go on to show that there exist some schedule $\sigma$ of events, which from an indecisive configuration $C$, lead to a continuous cycle of going from indecisive configuration to indecisive configuration. Specifically, the authors show that by sufficiently delaying some event $e$, there always exist a transition from one indecisive configuration to another. Thus, there exist some schedule $\sigma$ where the system cannot decide upon any values and can therefore not reach any forward progress; the consensus algorithm does not have liveness. 

% talk about the result and what it shows


In search for practical consensus mechanisms, major work has been directed towards consensus algorithm which can circumvent this result \citep{RN46, PBFT_MIT, RN51, RN42}. Specifically, the FLP impossibility holds for the scenario of a deterministic consensus algorithm, providing both safety and liveness, in a fully asynchronous network with at least a single faulty nodes. Such, by removing any of these assumptions, the result do not hold. In practical settings however, safety, liveness, as well as fault tolerance are oftentimes seen as mandatory. Therefore, the only way to circumvent the results are related to altering the synchronicity assumption about the network or the determinism of the consensus algorithm. In particular, consensus models which are non-deterministic, i.e. introduce randomization, do not adhere to the result \citep{RN51}. 


\subsubsection{Synchrony, Partial Synchrony and Asynchrony}

Additionally, in order to avoid the impossibility result \citep{RN40}, one can make the assumption that the underlying communication network is synchronous; messages between peers are delivered within some known fixed upper bound $\Delta$. This oftentimes do not reflect reality however, as communication over the internet is susceptible to delays and network failure. Thus, synchrony may not be enforceable in practical systems, depending on the characteristics of the network.

\citet{RN46} introduce the aspect of a partially synchronous network. It creates a middleground between synchronous and asynchronous networks, in which the upper bound $\Delta$ do exist, but it may either be not known a priori or may not hold before a certain point of time (i.e. eventually synchronous). This is sufficient to circumvent the FLP impossibility result. It however poses challenges related to the design of consensus mechanisms; if the bound cannot be known a priori, the consensus algorithm must be able to function regardless of what actual value the bound takes. If the bound only holds eventually, after some point of time $T$, the consensus algorithm must be able to function before $T$. 

As mentioned in section \ref{subsub:FLP}, the FLP impossibility result only hold for deterministic consensus. Thus, randomized consensus models may still achieve consensus in asynchronous network, assuming no upper bound $\Delta$ on the message delay between peers in the network. 

Based of this, the timing assumptions made by a consensus algorithms can be categorized accordingly:

\textbf{Synchronous:} There exist a known fixed upper bound $\Delta$ on the message delay between peers within the network.

\textbf{Partial Synchronous:} Either of the following statements hold: \begin{enumerate}[i]

    \item There exist a upper bound $\Delta$ on the message delay between peers within the network, but it cannot be known a priori.
    \item There exist a upper bound $\Delta$ on the message delay between peers within the network, but it does not hold before an unknown point of time $T$.
\end{enumerate}

\textbf{Asynchronous}: There does not exist a known fixed upper bound $\Delta$ on the message delay between peers within the network.


\subsection{Security considerations in blockchain systems}

\label{subsec:security}



When designing a blockchain system, there are several security aspects to considers. \citet{RN17} and \citet{RN30} provide insight into some core security issues related to blockchain systems. This section describes several of the most central security considerations towards blockchain systems, based on their reviews.

The concept of \textit{consistency} in relation to a blockchain system refers to its ability to keep the ledger consistent across the participants of the network \citep{RN17}. As stated by the CAP theorem \citep{CAP}, a distributed system cannot guarantee strong consistency, availability and partition tolerance simultaneously. Blockchain systems may therefore utilize different approaches in terms of consistency. In particular, common approaches implemented by  blockchain system are strong consistency, ensuring that nodes keep the same ledger at all times, and eventual consistency, in which nodes may have differing ledgers at some specific point of time, but eventually become consistent. Here, strong consistency comes with the trade-off of reduced availability in the event of network partitioning, while eventual consistency introduce the need for conflict resolution, should there be a dispute regarding which ledger is correct. 

\textit{Tamper-Resistance}, in terms of a blockchain system, refers to the system's ability to ensure the integrity of the information stored in its ledger, during and after block generation \citep{RN17}. Specifically, when new blocks are propagated within the system, the system's nodes need to be able to assert the validity of the transactions contained within the block. Adversaries may in particular attempt to modify a transaction to be included in the new block, or transactions already part of the ledger. Both are conventionally avoided by the use of strong cryptographic mechanisms, utilizing secure hash functions to assess that the integrity of transactions and blocks are not compromised, as well as digital signatures, ensuring that the transaction's origin are who they claim to be. 


Essential to system is its requirements towards \textit{Byzantine Fault Tolerance}. In a trustless peer-to-peer network, some degree of Byzantine fault tolerance is needed, to protect against arbitrary or malicious behavior by network participants.  The degree may then again vary depending on the setting of the system, whether it is permissioned or permissionless. Commonly labeled as the \textit{51\% attack}, malicious actors have been conjectured to have the ability to override honest transactions in cryptocurrencies like Bitcoin or Ethereum, given a majority of the hashing power of the network. This is further applicable to traditional BFT consensus models, where the system commonly assumes a maximum number of faulty nodes $f$, providing implications on the total number nodes required for consensus, and thus the scalability of the model.  

Another common attack vector within P2P systems is the \textit{Sybil attack}, where malicious actors create multiple fake identities, attempting to increase their influence upon the network. This is elegantly addressed in Nakamoto's Proof-of-Work scheme \cite{Nakamoto_Bitcoin_POW}, linking voting power to hashing power, thus making Sybil attacks ineffective. It is also addressed in permissioned blockchain systems, requiring all participants of the network to be authenticated, linking each identity to real world entities. The attack is consequently especially relevant in permissionless settings. 

Related to cryptocurrencies like Bitcoin, there is the \textit{Double spend attack}. This specifically refers to the action of spending a single amount of currency twice, i.e. in two separate transactions. In Bitcoin, this is partially dealt with by ensuring the integrity of transactions and including digital signatures, ensuring that parties partaking in the transaction are who they claim to be. Furthermore, transactions are only assumed to be confirmed after $k$ succeeding blocks, making the chance of reversing a previously committed transaction small. However, since the system's consensus termination is probabilistic, the potential for a fork is still there, enabling a double spend attack. This is further highlighted through the \textit{Blockchain Anomaly} \citep{RN38}, showing the impossibility of guaranteeing that certain committed transactions will not be removed from the main chain in the future. 

% start at early point of blockchain. build blocks privately, can forge time stamps to allow quicker generation of blocks. Publish larger chain later, causing double spends.
Some blockchain systems may also be vulnerable to a \textit{Long-Range attack} \citep{RN55}. Related to other majority consensus attacks, instead of attempting to hijack $k$ block confirmation limit, the attacker forks the chain at a much earlier point. The alternative chain is then privately mined upon by the attacker. \citet{RN55} proposes that in some types of blockchain systems, e.g. earlier versions of the Ethereum client, the attacker can take advantage of the fact that they are the only entity contributing to the alternative chain, accelerating the rate in which blocks are generated. This can then be used to overtake the main chain, enabling double spend attacks. \citet{RN55} goes on to explain that blockchain systems may protect against such attacks by limiting the variability among alternative chains. 

Another possible attack, the \textit{P+ Epsilon attack}  \citep{RN54}, leverages non-altruistic participants in the attacker's favor. By promising to provide some kind of reward, denoted $\epsilon$, the attacker can align other participants' incentives according to their own, creating a dominant strategy within the network. This then allows the attacker to carry out their goals, despite not controlling a majority of the network themselves, assuming that altruists do not constitute a majority within the network. The attacker may later on not pay out the reward promised, reaping the profit of the attack all by themselves \citep{RN30}.  

The \textit{balance attack} constitutes another flavor of the double spend attack, allowing malicious actors to force double spend attacks despite an honest majority, given sufficient network delay. \citet{RN39} provide a theoretical analysis of the attack and demonstrate its feasibility through experimental results, utilizing the Corda blockchain platform. The attack provides a valid security concern regarding use of proof-of-work based consensus schemes in blockchain systems with considerable network delay. 

\textit{Border Gateways Protocol Hijacking} (BGP) involve an attacker taking control over parts of the Internet routing infrastructure utilized by the blockchain system \citep{RN53}. By controlling key parts of the routing mechanisms of the network, attacker may be able to both partition the network, isolating participants from communicating with their peers, as well as significantly delaying block propagation. \citet{RN53} goes on to demonstrate the feasibility of both types of attacks. Similar to that of a balance attack, this can be used to perform double spends in certain types of blockchain systems. 

Blockchain systems may also be susceptible towards \textit{distributed denial of service} (DDOS) attacks. In particular, if the consensus model is leader-based, the system's liveness may be threatened. By overloading the leader with incoming traffic, this may prevent them from carrying out the consensus algorithm and thus impact the transaction throughput of the system. Furthermore, DDOS attacks may have implications on the number of faulty nodes of the system. This may impact the consensus scheme directly, in the case of BFT algorithms. It may also impact it indirectly, by altering the distribution of available computational resources, shifting the balance of power in the case of Proof-of-Work based consensus algorithms. 

To conclude, the \textit{degree of centralization} of a blockchain system may impact its security. Within certain consensus models, centralizing power within a subset of the nodes have inherent risks. It may provide incentive for DDOS attacks, as powerful nodes have greater influence upon the network, thus increasing the impact of an attack. It may furthermore heighten the risk of collusion, reducing the number of nodes for an adversary to corrupt. This may then lead to potential abuse of power, in form of double spend attacks.

Additionally, \citet{RN17} propose the security properties of \textit{user anonymity}, \textit{transaction confidentiality} and\textit{transaction unlinkability}. These properties all relate to the privacy of participants partaking in the blockchain system, protecting their identity and the confidentiality of the data they commit to the blockchain. This may be of great benefit in the setting of financial system, e.g. a cryptocurrency like Bitcoin, in which lack of privacy may enable attacks against lucrative targets. In an authenticated setting, it may be less applicable. 

\autoref{tab:background_security_considerations} provides a brief summary of the security considerations discussed. In terms of the SCM setting, with a permissioned blockchain system affected by limited network throughput, Byzantine fault tolerance, BGP and DDOS susceptibility are deemed the most generally applicable security considerations. Given that participants in the system are authenticated, a Sybil attack can effectively be combated. Furthermore, in the case of immediate transaction finality, which is provided by several types of consensus algorithms, forking is not possible. Thus,  long-range, P+ epsilon and balance attacks are therefore only applicable to Nakamoto style consensus algorithms, having probabilistic transaction finality. Finally, considering an authenticated setting, aspects like user anonymity and transaction unlinkability are deemed not relevant, while transaction confidentiality may be desired. 


\todo{Remove this table, or extend the table to substitute the section}

\renewcommand{\arraystretch}{1.25}
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm}p{7cm}}
         Name & Description \\\hline
         Consistency & Which approach will the system utilize to ensure the consistency of the system's ledger?  \\
         Tamper-Resistance & Is the system able to ensure the integrity of the ledger? \\
         Byzantine Fault Tolerance & To which an extent do the system need to tolerate Byzantine faults, e.g. adversarial nodes?  \\
         Sybil attack & How will the system protect against malicious actors creating multiple fake identities, attempting to outvote an honest majority?  \\
         Double spend attack & How will the system prevent nodes spending the same currency for two separate transactions? Specifically related to cryptocurrency systems.  \\
         Long-Range attack & To which extent is the system vulnerable to Long-Range attacks; forking the blockchain at its genesis block and privately building an alternative chain?  \\
         P+ Epsilon attack & To which extent is the system vulnerable to P+ Epsilon attacks; taking advantage of the dominant strategy among network participants, leveraging non-altruistic participants against the system? \\
         Balance attack & To which an extent is the system vulnerable to balancing attacks; splitting the network into sub-networks, delaying transactions and performing double spend attacks? \\
         Border Gateways Protocol \hspace{0.5cm} Hijacking & How will the system handle adversarial attacks against the network's routing mechanisms; partitioning the network or delaying block propagation? \\
         DDOS susceptibility &  To which an extent is the system susceptible to DDOS attacks, in terms of impact upon safety and liveness? Especially relevant for leader based consensus models. \\ 
         Degree of centralization & To which an extent is the system centralized around a subset of participants? This may have implications on various double spend attacks, as well as DDOS susceptibility.   \\
         User anonymity & Are participants of the system able to partake in transactions while staying anonymous?\\
         Transaction confidentiality & To which extent are transactions kept confidential? \\
         Transaction unlinkability & To which extent is it possible to link a group of transactions to a specific identity?\\
    \end{tabular}
    \caption{Security considerations for blockchain systems}
    \label{tab:background_security_considerations}
\end{table}

==> sections/scenario.tex <==
%\section{Application scenario}
%\label{sec:app_scenario}
% Section will give insight into application scenario of blockchain technology and the specific scenario which we focus on in this paper.
%This section describes the specific application scenario we consider in our research; enterprise blockchain systems used within SCM, with low network throughput. Additionally, the limitations of the research are then described, based on the context of the application scenario.
%\subsection{Scenario}
%In this paper, we specifically envision an enterprise, permissioned blockchain system. The participants of the network are comparable to that of independent organizations, utilizing the blockchain system in a cooperative manner. 
We assume an authenticated setting, in which each node $N_i$ have established a cryptographic encryption key $Ek_{i,j}$ with their respective \textit{neighbors} $N_j \in N$ , before the execution of a round of consensus. Here neighbors refer to any node in which $N_i$ either need to send or receive messages from, in order to carry out a round of the consensus algorithm. Having established such an encryption key, a message passing between two nodes is assumed to be comparable to a single round-trip time, i.e. 1 RTT. 

A consensus algorithm's communication complexity is measured in terms of the number of bits sent, related to the number of nodes $n$ in the network. A round of consensus involves both reaching an agreement, as well as propagating necessary data within the network in order for all nodes $N_i \in N$ to be able to commit the decided block to their local ledger. Following this understanding, an optimal consensus algorithm in terms of communication complexity involves $\Omega(n)$ bits being sent each round.

Network nodes are assumed to be heterogeneous. In particular, nodes may have different computational and memory resources, use different communication protocols among each other, and have varying geographical distance between each other, contributing to the network latency. Furthermore, the network is assumed to possibly span a large geographical area, in which nodes may have widely varying network latency among each other. This latency may also change over time, e.g. a node corresponding to a vessel transporting goods may move closer to one of its neighbors, thus reducing the network latency among them. 

A particular constraint of the network are periods of limited network throughput. Specifically, the network's nodes $N$ are assumed to be either stable, denoted $N_s$, or unstable, denoted $N_u$. Unstable nodes are expected to experience periods of poor or no network connection, in contrast to stable nodes, which are expected to exhibit a consistent connection across consensus rounds. As an illustrating example, a stable node could correspond to an office building in a metropolitan area, having access to a high speed WLAN, while an unstable node could correspond to a vessel traveling international waters, where as access to the internet may vary during the vessel's voyage. 

\subsection{Limitations}

% permissioned - need way to govern network. Assume authenticated.

The scenario focus solely on a permissioned setting. Specifically, there is some administrative structure which governs who are allowed to participate in the network. Furthermore, we assume an authenticated setting. This limits the research in terms of public blockchain systems. In particular, the need for Sybil attack resistance is relaxed, as all participants of the network are authenticated and approved by the system. 

% low network throughput - 

A differentiating factor of the scenario is that the system is significantly affected by low network throughput. This increases the effect which communication related costs have on metrics such as transaction throughput. Furthermore, since a subset of the nodes may experience poor network throughput, the system may be especially asynchronous, compared to other scenarios. This limits the research to systems affected by such constraints. In particular, blockchain systems with stable network throughput may emphasize other considerations in terms of their consensus mechanisms, as communication costs become less significant.

% high latency - geograpically distributed
Finally, as the nodes of the network are distributed over a large geographical area, some nodes may experience high network latency in communicating with other nodes. This may significantly affect consensus mechanisms which rely on timing assumptions related to the network. The research is therefore limited to that of networks of scale; if a system's nodes are closer in distance, latency related costs may be negligible. 



